Searching for gravitational waves emitted by binaries with spinning components

In this thesis we consider the data analysis problem of detecting gravitational waves emitted by inspiraling binary systems. Detection of gravitational waves will open a new window on the Universe enabling direct detection of systems such as binary black holes for the first time. In the first Chapter we show how gravitational waves are derived from Einstein's General theory of Relativity and discuss the emission of gravitational waves from inspiraling binaries and how this radiation may be detected using laser interferometers. Around two thirds of stars inhabit binary systems. As they orbit each other they will emit both energy and angular momentum in the form of gravitational waves which will inevitably lead to their inspiral and eventual merger. To date, searches for gravitational waves emitted during the inspiral of binary systems have concentrated on systems with non-spinning components. In Chapter 2 we detail the first dedicated search for binaries consisting of spinning stellar mass compact objects. We analysed 788 hours of data collected during the third science run (S3) of the LIGO detectors, no detection of gravitational waves was made and we set an upper limit on the rate of coalescences of stellar mass binaries. The inspiral of stellar mass compact objects into super massive black holes will radiate gravitational waves at frequencies detectable by the planned space-based LISA mission. In Chapter 3 we describe the development and testing of a computationally cheap method to detect the loudest few extreme mass ratio inspiral events that LISA will be sensitive to.

==> Chapter3/LIGO_S3SBBH_v2.tex <==
%$Id: LIGO_S3SBBH_v2.tex,v 1.1.1.1 2007-10-26 15:41:51 spxgwj Exp $

%\chapter{Searching for spinning \bbhs in LIGO data}
%\label{ch:s3sbbh}

%{\bf estimate number of physical templates required}


\section{Development of detection template families to capture 
gravitational waves from spinning systems}

In the introduction we showed that the optimal method to detect a known
signal in a noisy data stream is to perform matched-filtering using
templates that accurately represent the signal weighted (in the 
frequency domain) by the power spectrum of the noise.
%
We cannot use the ``target model'' waveform as a detection template since 
the large number of parameters needed to describe the waveform 
(i.e., 17, or 15 if we assume circular orbits) 
mean 
that we would require an intractably huge number of templates to cover the 
parameter space 
(i.e., the range of masses, spin magnitudes and orientations \dots) 
we wish to search. 
As well as increasing the computational cost of the search, such a 
large number of templates would lead to an unnacceptably high rate of false 
alarms and decrease the statistical significance of any detection.
%
{\bf Introduce term DTF, fewer parameters etc.}
%
In Apostolatos (1995) \cite{Apostolatos:1995} Apostolatos introduces 
the fitting factor (FF) as a quantitative measure of how well a given 
family of templates
can ``fit'' a predicted gravitational waveform.  The value of the fitting 
factor gives the reduction in signal to noise ratio (SNR) 
caused by using a given detection template
family rather than the true signal. The distance-range of a search for 
gravitational wave signals emitted by astrophysical systems is limited by 
the lowest SNR for which a true signal can be disintinguished from noise.
Using a detection template family with a $FF=0.9$ would result in a $10\%$ 
drop in distance range and a corresponding $(1-0.9^3 \approx) 27\%$ drop 
in detectable event rate. Apostolatos measures low fitting factors when 
using non-modulated PN templates to search for a spin-modulated 
gravitational wave signal (Sec.~VIII of Apostolatos (1995) 
\cite{Apostolatos:1995}. Results from this analysis will be discussed
later in this section). 
These results clearly motivate the development of a detection template family 
which can accurately model the spin-induced modulation of the gravitational 
wave signal.
We will now review the analysis of the effects of precessing, 
inspiraling systems and see how this has informed the development of a new
detection template family designed to capture their gravitational wave
emission.

\subsection{Previous analysis on the effect of spin on gravitational waves}
%\subsection{Review of ACST \cite{ACST}}
%\subsection{Simple and transitional precession}
In ACST \cite{ACST} the authors consider a simplified form of the 
target model neglecting other post-Newtonian corrections in order 
to emphasise the effects of spin upon upon the systems dynamics and 
gravitational wave emission.
The authors concentrate their analysis on two special binary 
configurations; 
i) $m_{1} \simeq m_{2}$ which could represent a NS-NS system
or a symmetric BH-BH system and
ii) $\Sv_{2} = 0$ which could represent a very
assymetric system ($m_{1} \gg m_{2}$) for which the spin of the 
lower mass component could be neglected.
For case i) the authors make the additional assumption that spin-spin 
effects can be ignored since they occur at a higher 
post-Newtonian order (2PN), and therefore typically be smaller 
than the leading spin-orbit term (1.5PN). Spin-spin effects
cannot of course for a system with only one spinning component
as in case ii). 
Making the assumptions described the authors were able to write the
precession equations as
\begin{eqnarray}
\label{S1ACST}
\dot{\hat{\Sv}}_{1} &=&
\left(
2 + \frac{3 m_{2}}{2 m_{1}}
\right) \frac{\Jv}{r^{3}}  \times \hat{\Sv}_{1} \\
\label{LNACST}
\dot{\hat{\Lv}}_{N} &=& 
\left(
2 + \frac{3 m_{2}}{2 m_{1}} 
\right)
\frac{\Jv}{r^{3}}
\times \hat{\Lv}_{N}
\end{eqnarray}
where $\Sv = \Sv_{1} + \Sv_{2}$.
\footnote{To derive these simplified precession equations take the precession 
equations given in Eq.~(11) of ACST \cite{ACST} and neglect all
spin-spin and higher order terms. 
We use the result that $\Jv \times \Lv 
= (\Lv+\Sv) \times \Lv 
= (\Lv \times \Lv) + (\Sv \times \Lv)$
which reduces to $\Jv \times \Lv = \Sv \times \Lv$
(and similarly $\Jv \times \Sv = \Lv \times \Sv$) to write the
right hand side of the simplified precessional equations in terms of
$\Jv$.}
For these {\it ACST configurations} the authors constructed approximate
solutions to the precession and inspiral equations and were able to gain
insight into the dynamics of these binary's during their inspiral.

The authors identify two distinct evolutionary behavours of the binary: 
i) {\it simple precession} occurs when total angular momentum $J>0$ and 
the orbital angular momentum $\Lv_{N}$ and the spin angular momentum $\Sv$ 
precess about a near constant $\Jv$,
ii) {\it transitional precession} occurs when $\Lv$ and $\Sv$ are 
anti-aligned and of the same approximate magnitude such that $\Jv \sim 0$ 
and the system temporarily ``loses its gyroscopic bearings and tumbles in 
space''.
As discussed previously during the course of inspiral $|\Sv|$ will remain
almost constant while $|\Lv|$ will reduce with time. Therefore, for 
transitional precession to occur we require that 
initially $|\Lv| > |\Sv|$ and that $\Lv$ and $\Sv$ be
approximately anti-aligned with each other.
The evolution of orbital $\Lv$, spin $\Sv$ and total angular momentum
$\Jv$ during simple and transitional precession is shown in
Fig.~\ref{fig:simple_transitional}.
Considering the simplified precession equations (Eqs.~(\ref{S1ACST}) and
(\ref{LNACST})) we can show that $\Lv$ and $\Sv$ maintain fixed directions
relative to each other as they precess about $\Jv$ which we can express
as 
\begin{eqnarray}
\label{kappa}
\kappa \equiv \hat{\Sv} \cdot \hat{\Lv}
\end{eqnarray}
where $\kappa$ will be a constant of the motion. 
\footnote{To prove that $\equiv \hat{\Sv} \cdot \hat{\Lv}$ is a constant of
the motion consider the time derivative 
$\dot{(\hat{\Sv} \cdot \hat{\Lv})} =
\hat{\Sv} \cdot \dot{\hat{\Lv}} + \hat{\Lv} \cdot \dot{\hat{\Sv}}$.
When evaluating the two terms on the right hand side both will contain
cross products of a vector with itself and therefore be equal to zero.}
The opening angle $\rm{cos}^{-1} \kappa$ between $\Lv$ and $\Sv$ 
will remain constant throughout the inspiral. 
During inspiral $|\Lv|$ and $|\Jv|$ will reduce while $|\Sv|$ remains 
approximately constant. From Fig.~\ref{fig:simple_transitional} we
see that these conditions will cause the opening angle $\lambda_{L}$ 
between $\Lv$ and $\Jv$ to increase with time during the inspiral. 

The random nature of the motion of $\Jv$ during transitional precession
makes the accurate prediction of the resulting waveform practically
impossible and it is therefore fortunate that most inspiral evolutions
do not exhibit transitional precession {\bf reference this}.

\begin{figure}
\begin{center}
\includegraphics[angle=0, width=0.7\textwidth]{Chapter3/simple_transitional.pdf}
\caption{The evolution of orbital $\Lv$, spin $\Sv$ and total angular momentum
$\Jv$ during simple and transitional precession.
In case i) only simple precession occurs as the total angular momentum $\Jv$ 
remains relatively large and roughly constant in direction while $\Lv$ 
and $\Sv$ precess about it.
In case ii) the evolution undergoes simple precession at early times ($t_{1}$)
until at around $t_{2}$, $\Lv$ has become similar in magnitude to $\Sv$ 
leading such that $\Jv = \Lv + \Sv \sim 0$. The system will undergo a
period of transitional precession, during which the system
will tumble randomly in space, until $|\Sv| > |\Lv|$ and simple
precession is resumed ($t_{3}$).
This figure is based upon Fig.~2 of ACST \cite{ACST}.
}
\label{fig:simple_transitional}
\end{center}
\end{figure}

From the simplified precession equations (Eqs.~(\ref{S1ACST}) and 
(\ref{LNACST})) we see that during simple precession 
$\Lv$ and $\Sv$ will precess about $\Jv$ with angular frequency 
\begin{eqnarray}
\Omega_{p} = 
\left(
2 + \frac{3 m_{2}}{2 m_{1}} \frac{\Jv}{r^{3}}
\right) = \frac{d \alpha}{dt}
\end{eqnarray}
where we have also defined the precession angle $\alpha$ 
(see Fig.~\ref{fig:orbangmmtm_cone}). 
The authors of ACST \cite{ACST} considered cases where 
$\Lv \gg \Sv$ and where $\Sv \gg \Lv$ and found that the
evolution of the precession angle could be approximated by
a power law in orbital frequency $f = \omega/ 2\pi$:
\footnote{Please note that an error occurs in the first bracketed terms of
the right hand side of Eq.~(45) of \cite{ACST}. The term $1+3M_{1}/4M_{2}$
should in fact read $1+3M_{2}/4M_{1}$ and appears correctly in Eq.~(29)
of \cite{Apostolatos:1995}.})
\begin{displaymath}
\label{alphaf}
\frac{\alpha(f)}{2 \pi} \simeq
\left\{
\begin{array}{ll}
11 
\left(    
1 + \frac{3 m_{2}}{4 m_{2}} 
\right)
\frac{10 M_{\odot}}{M} \frac{10 {\rm{Hz}}}{f}
& \rm{for} \, \Lv \gg \Sv \\
1.9 
\left(
1 + \frac{3 m_{2}}{4 m_{2}} 
\right)
\frac{m_{1}}{m_{2}} \frac{S}{m_{1}^{2}} 
\left( \frac{10 M_{\odot}}{M} \frac{10 {\rm{Hz}}}{f}
\right)^{2/3}
& \rm{for} \, \Sv \gg \Lv. 
\end{array} 
\right.
\end{displaymath}
%Comparing $\alpha(f) / 2\pi$ at differen 

\begin{figure}
\begin{center}
\includegraphics[angle=0, width=0.7\textwidth]{Chapter3/orbangmmtm_cone.pdf}
\caption{During simple precession the orbital angular momentum $\Lv$ 
of the (ACST configuration) binary will precess about the total angular
momentum $\Jv$ with frequency $\Omega_{p}$. The opening angle $\lambda_{L}$
and the precession angle $\alpha$ are also identified.
This figure is based upon Fig.~4 of ACST \cite{ACST}.
} 
\label{fig:orbangmmtm_cone}
\end{center}
\end{figure}

In Apostolatos (1995) \cite{Apostolatos:1995} introduces 
the fitting factor (FF) as a quantitative measure of the reduction of SNR 
caused by using a particular family of templates in order 
to capture a predicted gravitational
waveform.
The fitting factor is given as
\begin{eqnarray}
{\rm{FF}} = 
{\rm{max}}_{\lambda_{1}, \lambda_{2} \dots} 
\frac{\left< h, T_{\lambda_{1}, \lambda_{2} \dots} \right>}
{\sqrt{  
\left< h, h  \right> 
\left< T_{\lambda_{1}, \lambda_{2} \dots}, 
T_{\lambda_{1}, \lambda_{2} \dots} \right>
}}
\end{eqnarray}
where $h$ is our best prediction of the gravitational waveform that will
be observed and $T$ is a template designed to capture $h$ and which is
parameterised by $\lambda_{1}, \lambda_{2} \dots$.
The denominator ensures that $0 leq {\rm{FF}} leq 1$.
In this paper Apostolatos writes the detector response to a precessing,
inspiraling binary as
\begin{eqnarray}
\tilde{h}_{\rm{resp}}(f) \simeq 
\frac{1}{2} \tilde{h}_{C}(f) \times {\rm{AM}} \times {\rm{PM}}
\end{eqnarray}
where $\tilde{h}_{C}(f)$ is a non-modulated carrier signal and
AM and PM represent amplitude and phase modulations caused by
spin-induced precession (see Eq.~(17) of Apostolatos (1995) 
\cite{Apostolatos:1995} and note that the final multiplucative
factor is approximately unity).
Apostolatos investigates the relative influence of phase and 
amplitude modulations upon the fitting factor
when the templates used to detect spin-modulated gravitation
waves do not themselves include the effects of spin.
It was found that
at worst, amplitude modulation alone can only account for
fitting factors dropping to $\sim 0.9$ whereas phase modulation
can can the fitting factor to drop to below $0.6$.

Apostolatos also investigated the effect of the opening angle between
spin and and orbital angular momentum (i.e., $\cos^{-1} \kappa$) 
on the fitting factors.
When considering a maximally spinning $10M_{\odot}$ BH and a non-spinning
NS $FF < 0.9$ were measured for around a quarter of systems with a
$\cos^{-1} \kappa = 30^\circ$.
When the opening angle is increased to $\cos^{-1} \kappa = 140^\circ$ 
then $FF < 0.9$ are measured for nearly all systems.
%It is seen that the
%FF reduces as the opening angle of the precession cone
%$\lambda_{L} = {\rm{cos}}^-1 \hat{\Lv}_{N} \cdot \hat{Jv})$
%increases. If the opening angle between $\Lv$ and $\Jv$ is small then
%$\lambda_{L}$ will be small and FFs should be high regardless of the binary's
%component masses.

Building on work in ACST \cite{ACST}, Apostolatos suggests in 
\cite{Apostolatos:1995, Apostolatos:1996} that the spin-induced modulational 
effects of the gravitational wave signal's phase be captured by adding 
modulational terms to the standard non-modulational (NM) frequency domain 
phasing of templates used to search for the inspiral of binaries with 
non-spinning components (see Eq.~(12) of Apostolatos (1996)) 
\cite{Apostolatos:1996}):
\begin{equation}
\label{apostansatz}
\psi_{\rm{Spin-Modulated}}(f) \rightarrow \psi_{\rm{Non-Modulated}}(f) + 
\mathcal{C} (\delta + \mathcal{B} f^{-2/3}).
\end{equation}
This is the Apostolatos ansatz.
It makes sense that the modulational term occurs at $f^{-2/3}$ since this 
corresponds to the power law evolution of the precession angle when 
$S \gg L$ (see Eq.~(\ref{alphaf})). 
% more on freq dependence, apost:1996 also tests f^-1...
An implementation of this detection template family 
(which we shall refer to as the Apostolatos family) was tested in 
\cite{Grandclement2003} but ...

\section{BCV2 analysis of spinning binary systems}
\label{BCV2analysis}
In BCV2 the authors used the target model described in 
Sec.~\ref{Sec:TargetModel} to further investigate the effects of spin
upon the observed gravitational waveform which lead to the development
of a new detection family family (which we shall refer to as the
BCV2 DTF).
The BCV2 analysis considers a wider range of systems than ACST and do
not limit themselves the ACST configurations previously discussed
(i.e., either $m_{1} \simeq m_{2}$ or $\Sv_{2} = 0$).
In BCV2 the authors consider BH-BH systems with masses
$(20,10)M_{\odot}$,
$(15,15)M_{\odot}$,
$(20,5)M_{\odot}$,
$(10,10)M_{\odot}$ and
$(7,5)M_{\odot}$
consisting of maximally spinning BHs
and NS-BH systems with masses 
$(1.4,10)M_{\odot}$ consisting of a maximally spinning BH and a
non-spinning BH. 
{\bf angles? VIB, VIC... }
We shall refer to these as {\it BCV2 configurations}.
The choices of spin are not based upon astrophysical results
(most of the spin measurements summarised earlier were published after
BCV2 \cite{BCV2}) but to emphasise the effects of spins upon the
evolution and emission of these systems.
We summarise the findings of their analysis here.

When ignoring spin-spin coupling (but still considering binaries
consisting of two spinning bodies) the authors of BCV2 \cite{BCV2}
find a generalisation of Eq.~(\ref{kappa}) for the opening angle
between the orbital angular momentum and the spins:
\begin{eqnarray} 
\kappa_{\rm{eff}} \equiv 
\frac{\hat{\Lv}_{N} \cdot \Sv_{{\rm{eff}}}}
{M^{2}}
\end{eqnarray}
where we have defined an {\it effective spin}
\begin{eqnarray}
\Sv_{{\rm{eff}}} \equiv 
\left(1 + \frac{3 m_{2}}{4 m_{1}} \right) \Sv_{1} +
\left(1 + \frac{3 m_{1}}{4 m_{2}}   \right) \Sv_{2}. 
\end{eqnarray}
{\bf prediction of ending freq using kappa...}

The authors of BCV2 \cite{BCV2} investigate the regularity that 
transitional precession occurs.
They find an upper limit on the symmetric mass ratio 
$\eta \leq 0.22$
such that the system can evolve so that the magnitude
of the orbital momentum can decrease to 
$|\Lv_{N}| = |\Sv| \leq |\Sv_{1}| + |\Sv_{2}|$ 
before the system plunges (here, implicitly approximated
to occur at the Scwarschild radius, see Sec.~IIIE of
BCV2 \cite{BCV2} for the full description of this analysis
\footnote{There appears to be an error in
Eq.~(59) of BCV2 \cite{BCV2} in which both inequalities
should be reversed. 
In the first case we should demand that the minimum frequency 
for transitional precession to be possible $f_{\rm{trans}}^{\rm{min}}$
be less than the Scwarschild frequency $f_{\rm{Schw}}$ which would
lead to $f_{\rm{trans}}^{\rm{min}} / f_{\rm{Schw}} \leq 1$ and therefore
$\eta \leq 0.22.$}
).  

The authors of BCV2 \cite{BCV2} also investigated the effects of the spin
terms in the evolution of angular frequency (see Eqs.~(\ref{omegadot}), 
(\ref{omegadot1.5PN}) and (\ref{omegadot2PN})) 
on the accumulated orbital phase $\Psi$ (Eq.~\ref{accorbphase}).
They find that the effects of spin on the accumulated orbital phase $\Psi$
would be largely non-modulational and could be well captured by the 
phasing used to describe binaries with non-spinning components.
It is important to acknowledge that although the accumulated orbital
phase $\Psi$ is not modulated by the effects of spin that the phase (and 
amplitude) of the gravitational waveform observed at the detector
will be modulated by the spin-induced precession of the orbital plane
and that these effects should not be neglected. 
The phase $\Phi_{S}(t)$ which enters the general expression for detector
response $h_{\rm{resp}}$ (see Eq.~(\ref{hrespfinal})) is measured with respect 
to basis vector $\ev_{1}$ which is always in the instantaneous orbital plane 
(i.e., $\Lv_{N}(t) \cdot \ev_{1}(t) = 0$). 
In general $\Phi(t) \neq \Psi(t)$ since $\ev_{1}$ (and also $\ev_{2}$)
can have arbitrary rotation about $\Lv_{N}$.
In BCV2 \cite{BCV2} the authors define a new {\it precessing convention}
for the basis $\ev_{1,2}$ such that $\Phi(t) = \Psi(t)$ which allows the use
of $\Psi(f)$ when we write down the detector response $h_{\rm{resp}}$. From
their earlier observations we know that the non-modulational phase 
$\Psi_{NM}(f)$ used to describe the phasing of binaries with non-spinning
components is a good approximation to $\Psi$.

\section{The BCV2 detection template family for spinning systems}
\label{sec:BCV2dtf}
Following their analysis the authors of BCV2 \cite{BCV2}
proposed a detection template family representing a generalisation of 
the Apostolatos ansatz 
designed to capture gravitational waveforms from precessing, inspiraling
binaries in the adiabatic limit:
{\bf majority of terms can be found through maximisation}
From \cite{BCV2} Eq.~(86)
\begin{eqnarray}
\label{BCV2DTFa}
h( \dots; f) =
\left[ \sum_{k=1}^n (\alpha_k + i \alpha_{k+n}) 
\mathcal{A}_k (f) \right]
 e^{2 \pi i f t_{0}} e^{i \psi_{\rm{NM}} (f)}
\end{eqnarray}
for $f > 0$ and $h(f) = h^{*}(-f)$ for $f<0$. 
The $\alpha$'s represent the global phase, the strength of the amplitude 
modulation due to spin-induced precession, the relative phase of these 
modulations to the leading order amplitude ($f^{-7/6}$) and the internal 
complex phase of the modulation \cite{BCV2}.
The (real) amplitude functions $\mathcal{A}_k$ depend on the precise form
of the template chosen.
The function $\psi_{\rm{NM}}$ is the non-modulated phasing of a non-spining
binary and is given as power series of gravitational wave frequency $f$:
\begin{eqnarray} 
\psi_{\rm{NM}}(f) = f^{-5/3} \left (   
\psi_{0} 
+ \psi_{1/2} f^{1/3}  
+ \psi_{1} f^{2/3}  
+ \psi_{3/2} f  
\dots
\right).
\end{eqnarray} 
We have discussed in Sec.~\ref{BCV2analysis} that the non-modulated phase
$\Psi_{\rm{NM}}$ used to describe a binary with non-spinning components 
has been to capture well the accumulated orbital phase of binaries will
spinning components. 
In practise we find that the $\psi_{0}$ and $\psi_{3/2}$ terms dominate
and we neglect the other terms in this expansion.

In BCV2 \cite{BCV2} the authors suggest and test three forms of the
detection template family before recommending the third family which they
refer to as $(\psi_{0}, \psi_{3}, \beta)_{6}$ (Eq.~(90) of  BCV2 \cite{BCV2}):
\begin{eqnarray}
\label{BCV2DTF}
(\psi_{0}  \psi_{3} \beta)_{6}: && \nonumber \\
h(\dots; f) &=& f^{-7/6} 
\big[ 
  (\alpha_{1} + i\alpha{2})
+ (\alpha_{3} + i\alpha(4)) \cos(\beta f^{-2/3})
+ (\alpha_{5} + i\alpha(6)) \sin(\beta f^{-2/3})
\big] \nonumber  \\
&&\theta(f_{\rm{cut}} -f) 
e^{2 \pi i f t_{0}}
\rm{exp} i \big[ 
\psi_{0} f^{-5/3} + \psi_{3} f^{-2/3}
\big]
\end{eqnarray}
Rewriting Eq.~(\ref{BCV2DTF}) similarly to Eq.~(\ref{BCV2DTFa}) we find 
the three real 
amplitude functions, $\mathcal{A}_k(f_{\rm{cut}},\beta;f)$:
\begin{eqnarray}
\label{amp}
\mathcal{A}_1(f_{\rm{cut}},\beta;f) &=& f^{-7/6} 
\theta (f_{\rm{cut}}-f) \nonumber\\
\mathcal{A}_2(f_{\rm{cut}},\beta;f) &=& f^{-7/6} 
\cos(\beta f^{-2/3}) \theta (f_{\rm{cut}}-f) \nonumber\\
\mathcal{A}_3(f_{\rm{cut}},\beta;f) &=& f^{-7/6} 
\sin(\beta f^{-2/3}) \theta (f_{\rm{cut}}-f).
\end{eqnarray}.
The $\beta$ parameter varies to capture the effects of spin modulation.
We see that in the Apostolatos ansatz Eq.~(\ref{apostansatz}) the final
term in the cosine ($\beta f^{-2/3}$) is an approximation for the 
precession angle $\alpha$ when $\Sv \gg \Lv$ (see Eq.~(\ref{alphaf})). 
The parameter $\beta$ takes a similar role here. 
In Buonanno et al. (2005) \cite{PBCVT} (known as PBCVT) the authors
provide some physical interpretation of the $\beta$ parameter identifying
it as representing the rate of change of the precession angle $\alpha$, i.e.,
$\Omega_{p} = d \alpha / dt$ at the frequency band of good detector
sensitivity. 

The function $\theta$ is the Heaviside step function which is defined as
\begin{displaymath}
\theta(x) = \left\{
\begin{array}{cl}
 0  & x < 0 \\
 1  & x \geq 0
\end{array} \right.
\end{displaymath}
The parameter $f_{\rm{cut}}$ is used to cut the template when we no
longer have confidence that the template will provide a good match to
the signal (i.e., at the late stages of inspiral when the adiabatic 
approximation is no longer valid).
For gravitational wave frequency $f \leq f_{\rm{cut}}$ 
then $\theta(f_{\rm{cut}}-f) =1$.

The authors measured the fitting factor of this detection template family
{\bf finish this off}

\subsection{Maximisation of overlap over extrinsic parameters}
\label{sec:maximisation}
(BCV2 \cite{BCV2} Sec.~V A)\\
When listing the parameters used to describe a binary system consisting 
of spinning components we divided the parameters into two categories:
{\it intrinsic} parameters which describe properties of the system itself 
(e.g., masses, spins) and {\it extrinsic} parameters which describe the 
observers relation to the system (e.g., amplitude of observed emission, 
inclination and polarization angle).
Now considering the problem of finding the template $h$ within our DTF 
(as given in Eq.~(\ref{BCV2DTFa})) which yields the highest overlap with 
a given target signal $s$, we find that we can usefully separate the 
parameters used to describe our templates into these categories.
For the extrinsic parameters used to describe the templates (e.g.,
$\psi_{0}$, $\psi_{3}$, $\beta$ and $f_{\rm{cut}}$) we must construct
templates corresponding to each set of these parameters we wish to 
search for {\bf make this better!}.
Conversely, we are able to search automatically through the range of our 
intrinsic parameters (e.g., $t_{0}$ and $\alpha_{1 \dots 6}$) for the 
values which yield the best overlap.

(BCV1 \cite{BCV1} Sec.~II B)\\
To begin with we will consider the maximisation of the overlap over time.
The overlap between a time-shifted template $h(t-t_{0})$ and a signal $s$
is given by
\begin{eqnarray}
\left< s,h(t-t_{0}) \right> = 
4 \Re
\int_{0}^{\infty}
\tilde{s}^{*}(f) \tilde{h}(f) e^{2 \pi i f t_{0}}
\frac{df}{S_{n}(f)}.
\end{eqnarray}
Note that in the case of no time-shift ($t_{0} = 0$) we re-obtain
the formulae for the inner product given in Eq.~(\ref{inner_real_BCV}).
Rather than evaluate the overlap separately for every value of $t_{0}$ 
(in reality our time-series will be discretized so there will be a finite
number of values) we can employ the inverse Fourier transform to evaluate
all values of $t_{0}$ automatically. Finding the value of $t_{0}$ which 
maximises the overlap is simply a case of measuring the time that the maxima
in the resulting overlap time series occurs.

Now we shall consider the maximisation of the overlap over the $\alpha$
parameters.
Consider a template characterised only by its extrinsic parameters
$h(t_{0},\alpha_{k})$ which has been normalised such that the inner
product $\left<h,h\right>=1$. The overlap between the template $h$ and the 
signal $s$ is
\begin{eqnarray}
\max_{t_{0},\alpha_{k}} \left< s, h(t_{0},\alpha_{k}) \right>.
\end{eqnarray}
We find it expedient to orthonormalise our amplitude functions 
$\left< \widehat{\mathcal{A}}_{i}, 
\widehat{\mathcal{A}}_{j} \right> = \delta_{ij}$
and then define our {\it basis templates} as
\begin{eqnarray}
\label{basisTemplates}
\hat{h}_{k}(t_{0};f) &=& \widehat{\mathcal{A}}_{k} (f) 
e^{2 \pi i f t_{0}} e^{i \psi_{\rm{NM}}} \nonumber \\
\hat{h}_{k+n}(t_{0};f) &=& i \widehat{\mathcal{A}}_{k} (f) 
e^{2 \pi i f t_{0}} e^{i \psi_{\rm{NM}}}.
\end{eqnarray}
We are able to write our original template $h$ in terms of our
basis templates $\hat{h}_{k}$:
\begin{eqnarray}
h(t_{0},\alpha_{k};f) = \sum_{k=1}^{2n} \hat{\alpha}_{k} \hat{h}_{k}. 
\end{eqnarray}
The overlap between the template $h$ and a signal $s$ would be:
\begin{eqnarray}
\label{overlapBasis}
\max_{t_{0},\alpha_{k}} \left< s, h(t_{0},\alpha_{k}) \right> =
\max_{t_{0}} \max_{\hat{\alpha}_{k}} \sum_{k=1}^{2n} 
\hat{\alpha}_{k} \left< s, \hat{h}_{k}(t_{0}) \right>.
\end{eqnarray}
We will require that our templates be normalised and find that this
will lead to a constrain on the $\hat{\alpha}_{k}$ values 
\begin{eqnarray}
\left<h,h\right> &=& 1 \nonumber \\ 
&=& \sum_{k=1}^{2n} 
\left< 
\hat{\alpha}_{k} \hat{h}_{k},  
\hat{\alpha}_{k} \hat{h}_{k}  
\right> \nonumber \\
&=& \sum_{k=1}^{2n} \hat{\alpha}_{k}^{2} 
\left< \hat{h}_{k},\hat{h}_{k} \right> \nonumber \\
&=& \sum_{k=1}^{2n} \hat{\alpha}_{k}^{2}
\end{eqnarray}
where we have made use of the fact that since the amplitude functions
$\widehat{\mathcal{A}}_{k}$ are orthormal that the basis templates are
each orthonormalises,  $\left< \hat{h}_{i},\hat{h}_{j} \right> = \delta_{ij}$. 
We can find $\hat{\alpha}_{k}$ that maximise the overlap by employing the method
of Lagrange multipliers
\begin{eqnarray}
\Lambda = 
\sum_{k=1}^{2n} \hat{\alpha}_{k} \left< s, \hat{h}_{k}(t_{0}) \right>
 - \lambda \left[ \sum_{k=1}^{2n} \hat{\alpha}_{k}^{2} - 1 \right] 
\end{eqnarray}
which leads to
\begin{eqnarray}
\label{alphaHatMax}
\hat{\alpha}_{k} = 
\frac{ \left< s, \hat{h}_{k}(t_{0}) \right> }
{\sqrt{ \sum_{j=1}^{2n} \left< s, \hat{h}_{j}(t_{0}) \right> }}.
\end{eqnarray}
Substituting Eq.~(\ref{alphaHatMax}) into Eq.~(\ref{overlapBasis}) we find
the overlap maximised over $\hat{\alpha}_{k}$ 
\begin{eqnarray}
\max_{t_{0},\alpha_{k}} \left< s, h(t_{0},\alpha_{k}) \right> =
\sqrt{ \sum_{j=1}^{2n} \left< s, \hat{h}_{j}(t_{0}) \right> }.
\end{eqnarray}
In the case where the data to be filtered $x(t)$ contains both signal $s(t)$
and noise $n(t)$, i.e., $x(t) = n(t)+s(t)$ we can define the SNR as
\begin{eqnarray}
\label{BCV2SNR}
\rho = \max_{t_{0},\alpha_{k}} \left< x, h(t_{0},\alpha_{k}) \right> =
\sqrt{ \sum_{j=1}^{2n} \left< x, \hat{h}_{j}(t_{0}) \right> }
\end{eqnarray}


\subsection{Testing the detection template family}

We have just shown in Secs.~\ref{gaussianresponse}
and \ref{matchedfilterresponse} that when filtering 
data $x$ with a single template $h$:
\begin{itemize}
\item The output of filtering $\left<x,h \right>$ will be a Gaussian 
distributed variable if $x(t)$ is a Gaussian distributed variable. 
\item The expectation value of the $\left<n,h \right>$ will be zero if 
$\overline{n(t)} =0$.
\item The variance of $\left<n,h \right>$ will be unity if we use a 
normalised template such that $\left< h,h \right> =1$.
\end{itemize}

Therefore, for a Gaussian distributed variable $x$ with mean $0$ and variance
$1$, i.e. $x \sim N(0,1)$ we expect that $\left<x,h \right> \sim N(0,1)$.
Also, for a Gaussian distributed variable $x$ with mean $\mu$ and variance 
$\sigma^{2}$, i.e. $x \sim N(\mu,\sigma^2)$ we have
\begin{eqnarray}
\chi_{n}^{2} = \sum_{i=1}^{n} \frac{x_{i}^{2} - \mu_{i}} {\sigma_{i}^{2}}.
\end{eqnarray}
where $n$ is the number of degrees of freedom of the $\chi^2$ distribution.
The $\chi_{n}^{2}$ has mean $n$ and variance $2n$.

From Eq.~(\ref{BCV2SNR}) we see that 
\begin{eqnarray}
\rho^2 = \max_{t_{0},\alpha_{k}} \left< x, h(t_{0},\alpha_{k}) \right>^2 =
 \sum_{j=1}^{2n} \left< x, \hat{h}_{j}(t_{0}) \right>. 
\end{eqnarray}
For $x \sim N(0,1)$ we expect 
$\left< x, \hat{h}_{j}(t_{0}) \right> \sim N(0,1)$
and therefore that $\rho^2 \sim \chi_{2n}^2$ 
(using the range of $n$ used in the summation in this equation).

In general, when $\beta \neq 0$ we have 6 (non-zero) basis templates 
$\hat{h}_{j}$ and we would therefore expect $\rho^2 \sim \chi_{6}^2$.
When $\beta = 0$ we find that the (orthonormalised) amplitude functions
$\widehat{\mathcal{A}}_{2}$ and $\widehat{\mathcal{A}}_{3}$ become
zero at all frequencies.
Consequently we find that 4 of the 6 basis templates $\hat{h}_{j}$ 
defined in Eq.~(\ref{basisTemplates}) become zero at all frequencies.
Therefore we will expect that when $\beta = 0$, $\rho^2 \sim \chi_{2}^2$.
Figure \ref{fig:rhosq_hist} shows histograms of $\rho^2$ measured
using our detection template family (with $\beta = 0$ and $\beta \neq 0$)
when filtering Gaussian white noise with zero mean and unity standard
deviation. The response of our templates is as we would expect.

\begin{figure}
\begin{center}
\includegraphics[angle=0, width=0.45\textwidth]{Chapter3/GaussianHist_BetaZero_P.pdf}
\includegraphics[angle=0, width=0.45\textwidth]{Chapter3/GaussianHist_BetaNonZero_P.pdf}
\caption{Histograms of $\rho^{2}$ when $\beta = 0$ (left hand plot) and 
when $\beta \neq 0$ (right hand plot). As expected $\rho^2$ is distributed 
as a $\chi_{n}^{2}$ with the number of degrees of freedom $n$ equal to the number
of non-zero basis templates $\hat{h}_{i}$ used to calculate $\rho^{2}$.}
\label{fig:rhosq_hist}
\end{center}
\end{figure}

We also expect that for a normalised template $h$ that we would obtain an overlap
of unity if we were to use a template as our input data i.e.,$x = h$. 
Figure \ref{fig:wave_snr} shows the overlap measured (top plot) when we
perform this test. As expected an overlap of unity was measured.

\begin{figure}
\begin{center}
\includegraphics[angle=0, width=0.9\textwidth]{Chapter3/Wave_rhoSq_2005008_m1619_10_1000_P.pdf}
\caption{Plot showing the overlap ($\rho^2$) measured when filtering 
a template $h$ with itself. As expected we measure an overlap of unity
at the end time of the waveform.}
\label{fig:wave_snr}
\end{center}
\end{figure}

\section{Creating template banks}
\label{sec:templatebank}
{\bf we need to have a good and clear description of intrinsic and extrinsic
parameters before here...}

The detection template formula Eq.~(\ref{BCV2DTF}) describes a continous
multi-dimensional manifold containing every possible waveform that this
family can generate.
We can also imagine a manifold containing every possible gravitational
waveform we might observe from a binary with spinning components.
The parameters used to described the detection templates/signals 
act as the co-ordinates on these manifolds.
Figure \ref{fig:manifolds} shows the continous manifolds of signals and
templates.
We must now select a finite, discretely spaced subset of points on
the continous detection template manifold which will form the bank of 
templates we shall use to search for gravitational wave signals from 
binaries with spinning components.
There are two important decisions to be made in choosing the templates
for our bank: 
i) we must choose the parameter space we would like our template bank to
cover (i.e., the range of masses and spins of our target waveforms we are
interested in capturing)
and ii) the spacing of the templates within this region of parameter space
which will in turn directly influence the number of templates we will
have in our bank and the computational cost of the search.
We wish to space our templates as sparesly as possible (in order to minimize
the computational cost of the search) while also ensuring that we will
achieve good matches for any point on the continuous detection template 
manifold with one of the templates in the bank.
We will consider the question template spacing first.

\begin{figure}
\begin{center}
\includegraphics[angle=0, width=0.9\textwidth]{Chapter3/manifolds.pdf}
\caption{Schematic representation of the signal and continuous detection
template family manifolds as 2 dimensional surfaces.
The signal manifold (green) contains all the possible gravitational waveforms 
we might observe from a binary with spinning components.
The continuous detection template family manifold (blue) contains 
all the waveforms that can be represented by our 
detection template family Eq.~(\ref{BCV2DTF}).
We use the metric (of the intrinsic parameters, Eq.~\ref{tmpltbankmetric}) 
on the continous detection
template family in order to choose a finite set of templates (blue crosses)
which we refer to as our {\it template bank}.
We place the templates of our bank such that for any point chosen 
within the region  of the continous detection template family manifold 
we wish to cover an overlap (or match) greater than the specifed 
minimal match will be obtained with one of the templates in the bank. 
The fitting factor (previously discussed) describes the separation of
the signal and template manifolds. If the fitting factor was unity for
a region of parameter space the manifolds would be appear to touch in
that region. 
}
\label{fig:manifolds}
\end{center}
\end{figure}

\subsection{Calculating the metric on a continous detection template 
manifold}
Following the geometric formalism introduced in Owen (1996) \cite{Owen:1996}
we will find a metric on the manifold of continous detection template family
which will inform our choice of template spacing.
Our templates are parameterised by extrinsic parameters $\muv$ and intrinsic
parameters $\lambdav$, i.e., $h(\muv, \lambdav_{k})$ where $k$ is an index
which ranges through all the different extrinsic parameters $\lambdav$.

We consider two templates with slightly different parameters, 
$h(\muv, \lambdav_{k})$ and $h(\muv + \Delta \muv, \lambdav \Delta \lambdav)$
and calculate the match between them 
(from Owen (1996) \cite{Owen:1996} Eq.~(2.10)):
\begin{eqnarray}
M (\lambdav, \Delta \lambdav) \equiv 
{\rm{max}}_{\muv,\Delta \muv}
\left<
h(\muv, \lambdav),
h(\muv + \Delta \muv, \lambdav + \Delta \lambdav)
\right>.
\end{eqnarray}
We automatically maximise over the extrinsic parameters. 
Therefore the match describes the proportion of the optimal match (unity
for normalised templates) measured when using templates with intrinsic
parameters differing by $\Delta \lambdav$.
Expanding the match $M$ as a (Taylor) power series about 
$\Delta \lambdav = 0$ we find
\begin{eqnarray}
M (\lambdav, \Delta \lambdav) \simeq 
1 
+ \underbrace{\frac{\partial M}
             {\partial \Delta \lambda_{i}} \Delta \lambda_{i}}_{\sim 0} 
+ \frac{1}{2}
  \frac{\partial^{2} M}
  {\partial \Delta \lambda_{i} \partial \Delta \lambda_{j}} 
  \Delta \lambda_{i} \Delta \lambda_{j}
+ \dots
\end{eqnarray}
where we neglect the first derivative in this expansion since it will tend 
to zero around the maxima of $M$ at $\Delta \lambdav = 0$ and neglect terms 
beyond the second derivative. 
We define the metric on the intrinsic parameter space of the manifold of the 
continuous detection template family 
(from Owen (1996) \cite{Owen:1996} Eq.~(2.12)):
\begin{eqnarray}
\label{tmpltbankmetric}
g_{ij} (\lambdav) = - \frac{1}{2} \frac{\partial^{2} M}
  {\partial \Delta \lambda_{i} \partial \Delta \lambda_{j}}
  \Delta \lambda_{i} \Delta \lambda_{j}
\end{eqnarray}
for $\Delta \lambdav \sim 0$ which allows us to write the {\it mismatch} as
Owen (1996) \cite{Owen:1996} Eq.~(2.13)
\begin{eqnarray}
1 - M \simeq g_{ij} \Delta \lambda^{i} \Delta \lambda^{j}
\end{eqnarray}
We can use the metric $\gv$ to choose the largest spacings 
$\Delta \lambdav$ of our intrinsic parameters and still obtain matches 
greater than $M$ which we call the {\it minimal match}.

In Babak et al. (2006) \cite{babak:2006} the authors define the metric
in an alternative but usefully intuitive manner (see their
Eqs.(3.7)-(3.11)). 
The (proper) distance between two nearby templates 
separated by intrinsic parameters $\Delta \lambdav$
on the manifold is given by 
\begin{eqnarray} 
\left< h(\lambdav + \Delta \lambdav) - h(\lambdav), 
       h(\lambdav + \Delta \lambdav) - h(\lambdav) \right>   
\end{eqnarray}. 
Expanding the terms of the inner product we find that the (proper)
distance between these templates is
\begin{eqnarray}
\left< 
\frac{\partial h(\lambdav)} {\partial \Delta \lambda^{i}},
\frac{\partial h(\lambdav)} {\partial \Delta \lambda^{j}}       
\right>
\Delta \lambda^{i}
\Delta \lambda^{j}
\end{eqnarray}
from which, recalling Eq.~(\ref{spacetimemetric}) for the spacetime metric,  
it is natural to define the metric on the continuous detection template 
family as 
\begin{eqnarray}
g_{ij} (\lambdav) \equiv \left<
\frac{\partial h(\lambdav)} {\partial \Delta \lambda^{i}},
\frac{\partial h(\lambdav)} {\partial \Delta \lambda^{j}}
\right>
\end{eqnarray}.
These two definitions of the metric $g_{ij}$ are equivalent.

We will now describe the calculation of the metric for our detection
template and then the placement of templates using this metric.
This work was performed by Ben Owen and Chad Hanna for the 
Inspiral/CBC working group of the LSC.
The testing of the resulting template bank's coverage was
performed by Gareth Jones.

\subsection{Calculating the metric on the BCV2 continous detection 
template manifold}


\begin{itemize}
\item {\bf $f_{\rm{cut}}$}
\item We approximate the gravitational wave frequency of the 
last stable orbit (LSO) as the highest gravitational wave
frequency that would be emitted by test mass in Schwarschild
geometry:
\begin{eqnarray}
\label{fLSO}
f_{\rm{LSO}} = \frac{1}{6^{3/2} \pi M}.
\end{eqnarray}
\item Set $f_{\rm{cut}} = f_{\rm{LSO}}$. Over or under estimate??
\item See footnote 3 of Babak et al. (2006) \cite{babak:2006}, 
$f_{\rm{LSO}}$ depends only on mass...
\item Eq.~(3.6) of Allen et al. (2005) \cite{allen:2005}
$f_{\rm{ISCO}}$, difficult to determine except in the 
extreme mass ratio limit 
$\eta \rightarrow 0$, test mass orbiting a non-spinning 
(Schwarschild) black hole.  
\end{itemize}



\subsection{Template placement algorithm} 

\begin{figure}
\begin{center}
\includegraphics[width=0.9\textwidth]{Chapter3/FOMBANK_Multi_H1-754006846-2048.png}
\end{center}
\caption{A template bank generated with minimal match $= 0.95$
using 2048 seconds of H1 data taken during S3.
The crosses show the positions of individual templates in the
$(\psi_0,\psi_3,\beta)$ parameter space. For each template a value
for the cutoff frequency $f_{\rm cut}$ is estimated using Eq.~(\ref{fLSO}).
This bank requires a 3-dimensional template placement scheme in order
to place templates in the $(\psi_0,\psi_3,\beta)$ parameter space. Previous
searches for non-spinning systems have used 2-dimensional placement schemes.}
\label{fig:templatebank}
\end{figure}

\subsection{Testing the template bank}
\label{sub:testingbank}
The template bank was tested using a series of simulated signals
constructed using the equations of the target waveforms 
described in Sec.~\ref{Sec:TargetModel}.
We considered a variety of spin configurations including systems
where neither, one or both bodies were spinning.
We also considered masses outside the range we expected the template
bank to have good coverage in order to fully evaluate the range of masses
for which it could be used.
For each spin configuration we created a series of signals corresponding
to every mass combination: 
$1.0~M_{\odot} < m_{1}, m_{2} < 20.0~M_{\odot}$.
Using the initial LIGO design sensitivity we then measured the best
match that could be obtained for every signal using our template bank.
Figure~\ref{fig:banksims} shows a sample of the results from the tests of 
the template bank.
As expected we found that our template bank achieved the highest matches
for non-spinning (and therefore non-precessing) binaries. 
Performance degrades as spin-precessional effects become more pronounced 
i.e., when both bodies are spinning maximally with spins misaligned from 
the orbital angular momenta.
The template achieved matches $>0.9$ for a mass range 
%$[1-3]\times[12-20] M_{\odot}$.
$1.0~M_{\odot} < m_{1} < 3.0~M_{\odot}$ and
$12.0~M_{\odot} < m_{2} < 20.0~M_{\odot}$ 
(and equivalent systems with $m_{1}$ and $m_{2}$ swapped).
The detection template family (described in Sec.~\ref{sec:BCV2dtf}) is capable 
of obtaining high matches for comparable mass systems, the lower matches 
obtained for comparable mass systems are a result of targeting our template 
bank on asymmetric mass ratio systems 
(which are more susceptible to spin effects and conform to the strong 
modulation approximation). 

Matches below the specified minimal match of $0.95$ in the bank's region of 
good coverage are a consequence of (small) differences between the DTF and the 
target waveforms meaning that the DTF {\it cannot} perfectly match the target 
waveforms.

{\bf move some of the FF stuff earlier??}

The {\it fitting factor} (FF) measures the reduction of SNR due to differences 
between the DTF and the target waveform \cite{Apostolatos:1995} 
(and should not be confused with the minimal match which measures the loss of 
SNR due to discreteness of the template bank \cite{Owen:1996}).  
The DTF performance is evaluated and its fitting factor is measured 
in Sec.~VI of Ref.~\cite{BCV2}, 
for NS-BH systems an average FF of $\approx 0.93$ was measured 
\footnote{The authors of BCV2 \cite{BCV2} use a 
downhill simplex method called {\tt AMOEBA}\cite{NumericalRecipesInC} in 
order to obtain the best possible matches between the DTF and the target 
waveforms. 
This method works well for signals with high SNR but would not be effective 
in searching for weak signals in real detector data.}.

\begin{figure}
\begin{center}
\includegraphics[width=0.4\textwidth]{Chapter3/FOMINSPIRAL_bankSim_m1m2_contour_colour_000000.png}
\includegraphics[width=0.4\textwidth]{Chapter3/FOMINSPIRAL_bankSim_m1m2_contour_colour_000001.png} \\
\includegraphics[width=0.4\textwidth]{Chapter3/FOMINSPIRAL_bankSim_m1m2_contour_colour_AB1.png} 
\includegraphics[width=0.4\textwidth]{Chapter3/FOMINSPIRAL_bankSim_m1m2_contour_colour_AB2.png}
\end{center}
\caption{Plots showing the best match achieved by filtering a series of 
simulated signals through the template bank described in this section.
The values on the x and y axes correspond to the component masses of the 
binary source to which the simulated signal corresponds.
The colour of the plots shows the best match achieved for a given 
simulated signal.
The four subplots correspond to four different spin-configurations of the 
binary source. The top-left subplot shows results for a non-spinning 
binary system.  
The top-right subplot shows results for a system consisting of one 
non-spinning object and one maximally spinning object with its spin 
slightly misaligned with the orbital angular momentum. 
We would expect this system to precess.
The bottow two subplots show results for two generic precessing systems 
consisting of two maximally spinning bodies with spins and orbital 
angular momentum all misaligned from each other. 
We see that the region of the mass plane for which we obtain matches $> 0.9$ 
is largest for the non-spinning system and tends to be concentrated in the 
asymmetric mass region loosely bounded by 
$1.0~M_{\odot} < m_{1} < 3.0~M_{\odot}$ and
$12.0~M_{\odot} < m_{2} < 20.0~M_{\odot}$.}
\label{fig:banksims}
\end{figure}


\subsubsection{Estimating non-physical parameters in terms on physical 
parameters}
We are able to contruct approximate relationships between the physical 
parameters of our system $M$, $\eta$ and $\chi$ and the non-physical 
parameters used in the detection template family 
$\psi_0$, $\psi_3$ and $\beta$.

In Eq.~(3.3) and (3.4) of \cite{arun:084008} the phase of a gravitational 
wave inspiral is given to 3.5PN in the Fourier domain:
\begin{eqnarray}
\label{phase3.5PN}
\psi(f) &\equiv& \Psi_{f}(t_{f}) - \frac{\pi}{4} \nonumber \\
& = & 2 \pi f t_{c} - \phi_{c} - \frac{\pi}{4} + \frac{3}{128 \eta \nu^{5}} 
\sum_{k=0}^{N} \alpha_{k} \nu^{k}
\end{eqnarray}   
where $\nu = (\pi M f)^{1/3}$, $M=m_{1}+m_{2}$ and $\eta=m_{1} m_{2} / M^{2}$.
The dominant terms in this expansion correspond to 
\begin{eqnarray}
\alpha_{0} &=& 1 \\
\alpha_{3} &=& -16 \pi.
\end{eqnarray}
In \cite{BCV1, BCV2} we write the phase of our templates as:
\begin{eqnarray}
\label{psiNM}
\psi_{NM} = f^{-5/3}
(\psi_{0} + \psi_{1}f^{1/3} + \psi_{2}f^{2/3} + \psi_3{f}+...)
\end{eqnarray}
where it was noted that the phasing of the target model was captured well 
using only $\psi_{0}$ and $\psi_{3}$ in this expansion and setting the 
other $\psi$ coefficients
equal to zero. 

{\bf choose consistent notation for $\psi$'s}

If we equate coefficients in Eqs.~(\ref{phase3.5PN}) and (\ref{psiNM}) 
corresponding to the same order in frequency we find
\begin{eqnarray}
\psi_{0} &=& \frac{3}{128} \frac{1}{\eta (\pi M)^{5/3}} \\
\psi_{3} &=& \frac{-3}{8}  \frac{\pi^{1/3}}{\eta M^{2/3}}.
\end{eqnarray}

In \cite{ACST} we find that the evolution of the precessional angle 
$\alpha_{p}$  can be approximated by power laws of $f$ in 2 extreme 
cases; $\Lv \gg \Sv$ and $\Sv \gg \Lv$.
The first of these cases $\Lv \gg \Sv$ corresponds to a binary with either 
comparable masses or that is at the early stages of inspiral 
(i.e., large separation).
The second of these cases $\Sv \gg Lv$ corresponds to a binary with small 
mass ratio (i.e., large mass asymmetry) or that is at the late stages of 
inspiral (i.e., small separation) \cite{PBCVT}. 
In Fig.~(3) of \cite{kidder:821}, Kidder shows the evolution of $\Lv$ 
and $\Sv$ with separation $r$ for an equal
mass binary and a binary with a small mass ratio. 
This figure effectively illustrates the regimes during which 
the two extreme cases $\Lv \gg \Sv$ and $\Sv \gg \Lv$  are relevant.

When $\Sv \gg \Lv$ we find \footnote{Please note that a small error 
appears in Eq.~(45) of \cite{ACST}. 
The factors $1+ 3m_{1}/ 4m_{2}$ should in fact read $1+ 3m_{2}/ 4m_{1}$. 
Eq.~(42) of \cite{ACST} shows the correct factor as does \cite{PBCVT}.}.
\begin{eqnarray}
\alpha_{p}(f) \sim 3.8 \pi \left(1 + \frac{3}{4} \frac{m2}{m1}\right) 
\frac{m1}{m2} \chi 
\left(\frac{10 M_{\odot}}{M} \frac{10 Hz}{f}\right)^{2/3}.
\end{eqnarray}
We use the parameter $\beta$ as the coefficient in the power law, 
$\alpha_p(f) = \beta f^{-2/3}$ and thus find
that
\begin{eqnarray}
\beta \propto \left(1 + \frac{3}{4} \frac{m2}{m1}\right) \frac{m1}{m2} \chi
\left(\frac{10 M_{\odot}}{M} \right).
\end{eqnarray}
In the analysis of \cite{ACST} assume either that $m_{1} = m_{2}$ 
(meaning that spin-spin coupling can be ignored) 
or that $\Sv_{2} = 0$ which would correspond to systems with small 
mass ratio, e.g., the inspiral of a NS into a 
spinning BH.

{\bf asymetric mass systems $m_{1} \gg m_{2}$  can be modelled as systems 
with only a single body spinning since
even if both systems were spinning maximally $\Sv_{1} \gg \Sv_{2}$.}  

{\bf explain $\chi$}
Maximal value of $\beta$ occurs when $\chi = 1$.

Using the $f^{-2/3}$ power law approximation of $\alpha_{p}(f)$ is only expected 
to perform well matching binaries with $\Sv \gg \Lv$ but is shown to match well 
with systems with $\Lv \gg \Sv$ \cite{BCV2}.

\section{The data analysis pipeline}
\label{sec:pipeline}
The analysis of real detector data can be divided into a series of well 
defined processes with are collectively known as the 
{\it data analysis pipeline}.
Figure \ref{fig:pipeline} shows the data analysis pipeline
that was used for this analysis of LIGO data taken during its
third science run (S3).
The pipeline used for this search is the same as was used searches
for non-spinning binaries in S3 LIGO data. 
The searches for primordial black holes, binary neutron star and
binary black holes with non-spinning components using S3 and S4
LIGO data are described in Ref.~\cite{LIGOS3S4all}.

\begin{figure}
\begin{center}
\includegraphics[angle=0, width=0.9\textwidth]{Chapter3/pipeline.pdf}
\caption{Flowchart showing the various stages of the data analysis pipeline.
}
\label{fig:pipeline}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[angle=0, width=0.9\textwidth]{Chapter3/sciencesegment.pdf}
\caption{
Figure showing the subdivision of a science segment. 
This figure, originally produced by Duncan Brown, 
was reproduced from B. Abbot et al., Phys. Rev. D {\bf 72}, 082001 (2005) 
\cite{LIGOS2iul}, with permission from the authors. 
}
\label{fig:sciencesegment}
\end{center}
\end{figure}


\subsection{Data selection and the S3 LIGO data sample}

The matched-filter is found to be the optimal filter to find a
known signal in stationary and Gaussian noise. 
However, transients in the data due to problems with the detector or 
environmental disturbances can lead to a huge number of {\it false alarm}
triggers, i.e., triggers not caused by a true gravitational wave signal.
Stretches of data during which the detector had poor performance
or when there was an environmental disturbance will be excluded from
analysis. 
The study of the detector's behaviour is called detector characterisation.
The detector characterisation carried out on S3 LIGO data is detailed in
Christensen (for the LIGO Scientific Collaboration, 2005) \cite{S3Vetoes}. 

We categorise times when we know the detector had poor operation
with data quality (DQ) flags.
We construct a list of times for which each detector is 
operating well in what is known as {\it science mode} excluding times
associated with various DQ flags. 
We exclude times in which 
i) the detector was not collecting data ({\tt NO\_DATA}, {\tt NO\_RDS}),
ii) the interferometer was unlocked ({\tt UNLOCKED}), 
iii) there was invalid timing of the collected data ({\tt INVALID\_TIMING})
or iv) the data was not calibrated correctly i.e., missing calibration lines. 
({\tt CALIB\_LINE\_V03}).
For this search we have limited ourselves to data taken during LIGO's third
science run ({\tt OUTSIDE\_S3}).
The terms in brackets are the DQ flag names and the DQ flags listed here 
were used by all searches of S3 data.
As well as the use of DQ flags, later in the pipeline various short 
stretches of data will be vetoed. There are two types of vetoes: 
signal-based vetoes and detector-based vetoes, these will be discussed in more 
detail later.

Contiguous stretches of data taken when a detector is in science mode are
called {\it science segments}. 
Figure \ref{fig:sciencesegment} shows a single science segment and how it is
divided up for analysis.

The science segments are divided up into 2048 second {\it blocks}. 
Each block is divided into 15 overlapping 256 second 
{\it data segments}. Each data segment has 64 seconds overlap
with the preceeding and subsequent data segment (except for the
first and fifteenth data segment which only have one adjacent
data segment).
The power spectrum of each data segment is measured.
We then estimate the power spectrum of the block as the
median average of the power spectra of its 15 data segments.
To be clear, for each discrete frequency bin $f_{i} + \Delta f$ 
we will measure the power contained within it for each of the 15 
data segments and then take the median of these values to find 
the power for that frequency bin in the block's power spectrum.
The median average is used rather than the mean to avoid 
biasing of the average power spectrum by short-duration non-stationary
noise events in the data.

{\bf we FFT each data segment...}

There are two reasons we need to overlap data segments (and similarly
why we need to overlap 2048 second blocks).
This is discussed in detail in Allen et al. (2005) \cite{allen:2005}
and is briefly summarised here.
Firstly, the Fast Fourier Transform (FFT) we use in matched-filtering 
(see Sec. \ref{app:matchedfilter}) treats each data segment as
if it is periodic. The subsequent wrap-around effect causes a 
stretch of data the length of the template $T_{\rm{Template}}$ 
to be invalid at the start of each data segment.
Secondly, narrow lines (``spikes'') in the inverse noise power spectrum 
($S_{n}(f)^{-1}$) used in the inner product 
(see e.g., Eq.~(\ref{inner_real_BCV})) will cause corruption of data
throughout each data segment.
The inverse noise power spectrum is truncated in the time domain in order
to limit the corruption to stretches of data length $T_{\rm{Spec}}$ at the
start and end of each data segment. Note that we cannot choose 
$T_{\rm{Spec}}$ to arbitrarily small since that would effectively lose
important information about the (inverse) noise power spectrum in the
frequency domain.
These two effects lead to stretches of corrupted data of duration 
$T_{\rm{Template}} + T_{\rm{Spec}}$ at the beginning
and $T_{\rm{Spec}}$ at the end of each data segment.
In order to avoid corrupted data we
only analyse and record triggers from the central half (128 seconds) 
of each 256 second data segment and ignore the first and last 
quarters of each data segment. 
We then overlap each data segment with the preceeding and subsequent
data segment by 128 seconds to ensure all the data will be analysed.

At the end of a science segment it might be necessary to overlap
2048 second blocks by more than 128 seconds to ensure that we analyse as
much of the remaining data as possible. Care is taken to ensure that the
same stretch of data is not analysed twice.
Since it is not possible to overlap a 2048 second blocks at the very beginning
or end of a science segment, the first and last 64 seconds of  
each science segment will not be analysed.
Science segments shorter than 2048 seconds in duration will also not 
be analysed.

For each 2048 second block we will construct a template bank
which we shall subsequently use to filter it.
We do not analyse the first or last 64 seconds of each 2048 second 
block and we therefore overlap each block with the preceeding and
subsequent block by 128 seconds 
(except for the first and last block in the 
science segment which only have only have one adjacent block). 

\subsection{Playground data}
We specify a subset of our data to be {\it playground data} which
we use to tune various parameters (e.g., SNR thresholds, coincidence windows).
The use of playground data allows the data analyst to tune parameters while
remaining {\it blind} to the remainder of the data set thus avoiding  
statistical bias. 
The set of playground times is defined formally as
\begin{eqnarray} 
\mathcal{T} := 
\left\{ 
 \left[ t_{n}, t_{n} + 600 \right) : 
t_{n} = 729273613 + 6370 n, 
n \in \mathbb{Z}
\right\} 
\end{eqnarray} 
where $729273613$ is the GPS time of the beginning of LIGO's second
science run (from internal LIGO technical documents T030256 and T030020).
According to this definition playground times will account for, on average, 
$9.4\%$ of any given stretch of time.
Once parameters have been tuned using the playground data, the full data 
set (including playground) will be searched for gravitational wave
events. To avoid statistical bias, the values of the parameters chosen
after the analysis of playground data will remain fixed throughout the
subsequent analysis of the full data set.

Although it is possible to make a detection of a gravitational wave
during playground times, playground times are excluded from any 
upper limit calculations which are performed when no gravitational waves
have been detected.

\subsection{The S3 data set}
Data collected by the LIGO Hanford Observatory (LHO) detectors 
(i.e., H1 and H2) was only analyzed when both detectors 
were in science mode. This was due to concerns that since both of these 
detectors share the same vacuum system, the laser beam of a detector in 
anything but science mode might interfere with the other detector.

We denote periods of time when all three detectors are in science
mode as H1-H2-L1 times and periods when only the LHO detectors are on as
H1-H2 times. A coincident trigger consisting of a trigger in the H1 detector 
and the L1 detector will be referred to as an H1-L1 coincident trigger and 
similarly for other combinations of detectors.
In this search we analyzed 184 hours of H1-H2-L1 data and
604 hours of H1-H2 data (see Table \ref{tab:analysedtimes}).

We must also choose the lower frequency cutoff $f_{\rm{low}}$ which
will be the lower limit of any integrals we perform in the frequency domain 
(the upper frequency cutoff will depend on the particular template used and
the total mass of the source it represents {\bf ref earlier section}). 
There are competing factors that influence the choice of $f_{\rm{low}}$.
Binaries with larger masses will plunge and coalesce at lower frequencies
(see Eq.~{\ref{fLSO}}).
Taking lower values of $f_{\rm{low}}$ means that we will be sensitive to 
binaries with larger total mass and will also observe more orbital cycles
of inspiralling binaries in general. 
The observation of more cycles allows for greater SNR's to be achieved but 
would require longer duration templates to be produced which would increase 
the computational cost of the search.
Note that although increasing the mass range of a search to include heavier 
binaries will increase the number of template in the bank (for a given 
minimal match), the number of templates required to cover the higher-mass
region of parameter space is far smaller than the number of templates
required to cover the low-mass region. See, for example Fig.~5 of
Babak et al. (2006) \cite{babak:2006}.
However, at lower frequencies seimsic activity causes the detectors noise 
to become worse and the spectrum to be non-stationary
{\bf ref noise curve}. In practise we
take the lowest value of $f_{\rm{low}}$ for which the noise spectrum 
is approximately stationary. For S3 a value of $f_{\rm{low}} = 70 Hz$ 
was chosen. 
As the detectors achieve better sensitivity and greater stationarity of noise
lower values of $f_{\rm{low}}$ have decreased allowing higher mass binaries to
be searched for. 
In S4 and S5 searches lower cutoff frequencies as low as $f_{\rm{low}} = 40 Hz$
have been used. {\bf is this the lowest }

\begin{table}[htdp]
\caption{Summary of the amount of data analyzed in our various data sets. 
In S3 we only analyze data from the LHO detectors when both H1 and H2 are 
in science mode. Around $9.4\%$ of the data is classified as 
{\it playground data} and is used to tune the parameters of the search. 
Playground data is not included in the upper limit calculation but is 
still searched for possible detections. }
%\begin{ruledtabular}
\begin{tabular}{c|cc}
Data type & Total analyzed (hours) & Non-playground (hours) \\
\hline
H1-H2    & 604   & 548  \\
%H1-H2    & 604.0   & 547.7  \\
H1-H2-L1 & 184   & 167  \\
%H1-H2-L1 & 184.2   & 167.2  \\
\end{tabular}
%\end{ruledtabular}
\label{tab:analysedtimes}
\end{table}

\subsection{Template bank generation}
Using the estimated PSD we will calculate the template placement metric
Eq.~(\ref{tmpltbankmetric}) and create a template bank for each
2048s blocks of data for each detector (H1, H2 and L1).
The metric calculation and template placement scheme used in this
search is described in Sec.~\ref{sec:templatebank}.

In this search we use a minimal match of $0.95$.
Figure \ref{fig:FOMSize_VersusGPS_tmpltbank} shows the number of templates
in each template bank against GPS time for throughout S3.
We see a large increase in the size of the H2 template banks which was caused
by a flattening of the its power spectral density profile as S3 progressed.

\begin{figure}
\begin{center}
\includegraphics[angle=0, width=0.9\textwidth]{Chapter3/FOMSize_VersusGPS_tmpltbank.png}
\caption{Number of templates in each template bank. We generate a separate 
template bank for each 2048s block of data for each detector.
}
\label{fig:FOMSize_VersusGPS_tmpltbank}
\end{center}
\end{figure}

\subsection{Matched-filtering of detector data}
We matched-filter every 2048s block of data using each template in the associated 
template bank.
If the SNR measured by a particular template exceeds the SNR threshold
we record a trigger which contains details of the template and the time
at which the SNR threshold was exceeded.

For Gaussian white noise, $\rho^2$ will, in general, have a $\chi^2$ distribution 
with 6 degrees of freedom. 
In the case where the spin parameter $\beta = 0$ we find that 
$\mathcal{\widehat{A}}_2$ and $\mathcal{\widehat{A}}_3$
both vanish and that $\rho^2$ is described by a $\chi^2$ distribution with 
2 degrees of freedom.
To reflect the increased freedom we choose a higher SNR threshold, 
$\rho_{*} = 12$ when $\beta \neq 0$ and a lower value of
$\rho_{*} \approx 11.2$ when $\beta = 0$.
These values were chosen to give approximately the same number of triggers when 
analyzing Gaussian white noise and to ensure that the number of triggers produced 
during the real search was manageable.

\subsection{Coincident analysis}

\label{sub:coincAnalysis}
To minimize the false alarm probability and to increase the
significance of a true detection we demand that a gravitational wave
signal be observed by two or more detectors with similar parameters.
In order to determine whether a trigger measured by one particular detector 
should be considered as coincident with a trigger in another detector we 
define a set of coincidence windows.
In this search we demand that for triggers from different detectors to be 
considered as coincident they must satisfy the following conditions:
\begin{eqnarray}
|t_{1} - t_{2}| & < & \Delta t_{1} + \Delta t_{2} + T_{1,2}, \\
|\psi_{0,1} - \psi_{0,2}| & < & \Delta \psi_{0,1} + \Delta \psi_{0,2} \and \\
|\psi_{3,1} - \psi_{3,2}| & < & \Delta \psi_{3,1} + \Delta \psi_{3,2}
\end{eqnarray}
where $t_{i}$, $\psi_{0,i}$ and $\psi_{3,i}$ are the measured time of
coalescence and phenomenological mass parameters measured using our
template bank in detector $i$; 
$\Delta t_{i}$, $\Delta \psi_{0,i}$ and $\Delta \psi_{3,i}$
are our coincidence windows in detector $i$ and $T_{i,j}$ is the light 
travel time between detector locations $i$ and $j$. 
The light travel time between LHO and LLO is $\sim 10$ ms.

{\bf why use these parameters? what about beta, fcut, alphas...}

We tune our coincidence windows on the playground data in order to
recover as many of our simulated signals as possible whilst trying to 
minimize the false alarm rate.
The use of playground data allows us to tune our search parameters
without biasing the results of our full analysis.
The tuning method used for this and the non-spinning search on S3/S4
data is described fully in \cite{LIGOS3S4Tuning}.
Using this tuning method we find our coincidence windows to be equal for each
detector with values $\Delta t = 100$ ms,
$\Delta \psi_{0} = 40,000~ \rm{Hz}^{5/3} $  and
$\Delta \psi_{3} = 600~ \rm{Hz}^{2/3}$.
The value of $\Delta t$ used in this search is four times larger than the
$25$ ms value used in the S3 search for non-spinning binary black holes
\cite{LIGOS3S4all} indicating that the estimation of arrival time of a
gravitational waveform is less well determined in this search than in the
non-spinning search.

\begin{itemize}
\item Tuning of params using plotcoincwindow
\end{itemize}

\subsection{Background estimation}
\label{sub:background}
We estimate the rate of accidental coincidences, otherwise known as the
background or false alarm rate, for this search through analysis of
time-shifted data. We time-shift the triggers obtained from each detector
relative to each other and then repeat our analysis, searching for triggers
that occur in coincidence between 2 or more of the detectors. By choosing
our time-shifts to be suitably large
($\gg 10$ ms light travel time between LHO and LLO)
we ensure that none of the coincident triggers identified
in our time-shift analysis could be caused by a true gravitational wave signal
and can therefore be used as an estimate of the rate of accidental coincidences.
In practise we leave H1 data unshifted and time-shift H2 and L1 by increments
of $10$ and $5$ s respectively.
In this search, we analyzed 100 sets of time-shifted data
(50 forward shifts and 50 backward shifts).
For clarity we will use the term {\it in-time} to mean triggers which have not
been time-shifted.

\subsection{Combined SNR}
\label{sub:combSNR}
We assign a {\it combined signal-to-noise ratio} $\rho_{c}$ to our coincident 
triggers based upon the individual signal-to-noise ratios $\rho_{i}$
measured by each detector:
\begin{equation}
\label{combSNR_2ifo}
\rho_{c}^{2} = {\rm min} \left\{ \sum_i \rho_{\rm i}^2,
(a\rho_{\rm i}-b)^2 \right\}.
\end{equation}
In practise the parameters $a$ and $b$ are tuned so that the contours
of false alarm generated using Eq.~(\ref{combSNR_2ifo}) separate triggers generated
by software injection of simulated signals and background triggers
as cleanly as possible \cite{LIGOS3S4Tuning}(see the next subsection for details
of how we estimate the background). In this search we used values
$a = b = 3$ for all detectors. For coincident triggers found in all three
detectors we use:
\begin{equation}
\label{combSNR_3ifo}
\rho_{c}^{2} =  \sum_i \rho_{\rm i}^2.
\end{equation}

\begin{itemize}
\item bitten-L plots
\end{itemize}

\subsection{Vetoes}

\label{sub:vetoes}

\subsection{Instrument based vetoes}
We are able to veto some background triggers by observing correlation between 
the gravitational wave channel (AS\_Q) of a particular detector and one or 
more of its auxiliary channels which monitor the local physical environment. 
Since we would not expect a true gravitational wave signal to excite the 
auxiliary channels, we will treat as suspicious any excitation in the 
gravitational wave channel that is coincident in time with excitations in the 
auxiliary channels. 
A list of auxiliary channels found to effectively veto spurious 
(non-gravitational wave coincident triggers) were identified and used for all 
S3 searches \cite{S3Vetoes}.
%Additionally, another two
%auxiliary channels, L1:LSC-REFL\_Q and H1:LSC-MICH\_CTRL channels were 
%investigated as potential vetoes
%for this search.
%However the total amount of data discounted when using these channels as
%vetoes, known as the {\it dead-time}, was unacceptably large
%and it was decided not to use them in this search.
%Consequently, only the standard list of auxiliary channels were used to veto
%coincident triggers in this search.
Additional vetoes based upon other auxiliary channels were considered but were 
subsequently abandoned because the total amount of data these channels would 
have discounted, known as the {\it dead-time}, was unacceptably large.

\subsection{Signal based vetoes}
We can use the fact that the Hanford detectors are co-located to veto 
coincident triggers whose measured amplitude is not consistent between 
H1 and H2.
%We do not have an effective distance calculation for the triggers
%arising from this search but instead look
We check for consistency between the SNR values measured using H1 and H2 data 
for triggers found in coincidence. Since H1 is
%generally
the more sensitive instrument we simply required that the SNR measured in H1 
be greater than that measured in H2 for an event to survive this veto.
Since H1 and H2 were only operated when both were in science mode during S3, 
this veto means that there will be no H2-L1 coincident triggers since this 
would indicate that H2 had detected a trigger which H1 was unable to detect.

The $\chi^{2}$ veto used for the primordial black hole and binary neutron star
searches~\cite{LIGOS3S4all} has not not been investigated for use in searches 
using detection template families (i.e., this search and the S2-S4 searches for
non-spinning binary black holes \cite{LIGOS2bbh, LIGOS3S4all}).

% http://www.lsc-group.phys.uwm.edu/cgi-bin/enote.pl?nb=s3detchar&action=view&page=74
Veto categories 
\begin{enumerate}
\item Data Quality flags used in creation of {\it science segments}.
\item ``Unconditional vetoes''
\item ``Upper limit vetoes''
\item ``Conditional vetoes''
\end{enumerate}

\section{Results and follow-up analysis}
\label{sub:results}
In the search of the S3 LIGO data described in this paper, no triple-coincident
event candidates (exceeding our pre-determined SNR threshold and satisfying the
coincidence requirements described in Sec.~\ref{sub:coincAnalysis}) were found 
in triple-time (H1-H2-L1) data. 
Many double-coincident event candidates were found in both triple-time and 
double-time (H1-H2) data.

A cumulative histogram of combined SNR for in-time and background coincident 
triggers is shown in Fig.~\ref{fig:cum_hist}. 
We see that, at the SNR threshold (i.e., the leftmost points on this figure), 
the number of in-time double-coincident triggers is consistent with the number
of coincident triggers yielded by the time-shift analysis.
The small excess in the number of in-time H1-H2 coincident triggers at higher 
SNRs indicates that there is some correlation between the LHO detectors. 
The coincident triggers contributing to this excess have been investigated and 
are not believed to be caused by gravitational waves. 
Seismic activity at the Hanford site has been recorded throughout S3 and can 
cause data to become noisy simultaneously in H1 and H2.  
Coincident triggers caused by seismic noise will predominantly cause only 
in-time coincidences (although time-shift coincidences caused by two seismic 
events separated in time but shifted together can occur) leading to an excess 
of in-time coincident triggers as we have observed in Fig.~\ref{fig:cum_hist}.
As mentioned previously, there were no coincident triggers observed by all three 
detectors.

A scatter plot of the SNRs measured for coincident triggers in H1-H2 times
is shown in Fig.~\ref{fig:snr_snr}. The distribution of our in-time triggers 
is consistent with our estimation of the background. This is also true for
the double-coincident triggers measured in H1-H2-L1 times.
{\bf show these too?}

The loudest in-time coincident trigger was observed in H1-H2 when only the 
Hanford detectors were in science mode.
This event candidate is measured to have SNRs of 
$119.3$ in H1, 
$20.4$ in H2 
and a combined SNR of $58.3$.
The loudest coincident triggers are subjected to systematic follow-up 
investigations in which a variety of information (e.g., data quality at time 
of triggers, correlation between the detector's auxiliary channels and the 
gravitational wave channel) is used to assess whether the coincident triggers 
could be confidently claimed as detection of gravitational wave events.
This event is found at a time flagged for ``conditional'' vetoing. 
This means that during these times some of the detectors auxiliary channels 
exhibited correlation with the gravitational wave channel (AS\_Q ) and that 
we should be careful in how we treat event candidates found in these times.
For this particular coincident trigger an auxiliary channel indicated an
increased numbers of dust particles passing through the dark port beam
of the interferometer~\cite{S3Vetoes}.
Upon further investigation it was found that this coincident trigger occurred
during a period of seismic activity at the Hanford site and we
subsequently discounted this candidate as a potential gravitational wave event.
Time-frequency images of the gravitational wave channel around the time of this
candidate were inconsistent with expectations of what an inspiral signal should 
look like further reducing the plausibility of this candidate being a true 
gravitational wave event.
It is interesting, but unsurprising, to note that during the search for 
non-spinning binary black holes that also used S3 LIGO data, high-SNR triggers 
associated with this seismic activity were also detected \cite{LIGOS3S4all}.
Furthermore, the 20 next loudest event candidates were also investigated and 
none were found to be plausible gravitational wave event candidates.
Work is in progress to automate the follow-up investigative procedure and to 
include new techniques including null-stream and Markov chain Monte Carlo 
analysis for assessing the plausibility of coincident triggers as 
gravitational wave events. 

%\begin{figure}[hbtp]
%\includegraphics[width=0.5\textwidth]{H1H2times_plot_slide_trigs.png}
%\caption{The number of coincident triggers found in each time-shift of the H1-H2 time dataset.
%The solid horizontal line shows the mean number of coincident triggers measured across the
%time-shifts, the dashed lines show the one-sigma deviation from the mean.
%The number of in-time coincident triggers (time-shift number = 0, shown as a cross) is consistent 
%with the number of background coincident triggers (shown as pluses) and is within
%one-sigma of the mean number of coincident triggers.}
%\label{slide_trigs}
%\end{figure}

\begin{figure}
%[hbtp]
\begin{center}
\includegraphics[width=0.9\textwidth]{Chapter3/AllTimes_cum_hist_bitten_lsq}
\caption{
Cumulative histograms of the combined SNR, $\rho_{c}$ for in-time coincident triggers
(triangles) and our background (crosses with one-sigma deviation shown)
for all H1-H2 and H1-H2-L1 times within S3.
We see a small excess in the number of in-time coincident triggers with combined SNR
$\sim 45$. This excess was investigated and was caused by an excess of H1-H2 coincident
triggers. Since H1 and H2 are co-located, both detectors are affected by the same
local disturbances (e.g., seismic activity) which contributes to the number of in-time
coincidences but which is under-represented in time-shift estimates of the background.
}
\label{fig:cum_hist}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=0.9\textwidth]{Chapter3/H1H2times_H1_vs_H2_snr.png}
%\includegraphics[width=0.5\textwidth]{H1H2L1times_H_vs_L1_snr.png}
\caption{Scatter plot of SNR for coincident triggers in H1-H2 times. 
The light colored crosses represent in-time coincident triggers and the 
black pluses represent 
time-shift coincident triggers that we use to estimate the background. 
Note that due to our signal based veto on H1/H2 SNR
we see no coincident triggers with $\rho_{\mathrm{H1}} < \rho_{\mathrm{H2}}$.}
\label{fig:snr_snr}
\end{center}
\end{figure}

\section{Upper limit calculation}
\label{sub:upperlimit}
{\bf References
Biswas et al. (2007) \cite{ul},
Brady and Fairhurst (2007) \cite{systematics}
Brady et al. (2004) \cite{loudestGWDAW03}
}

Given the absence of plausible detection candidates within the search 
described above, we calculate an upper limit on the rate of
spinning compact object coalescence in the universe. 
We quote the upper limit rate in units of 
coalescences per year per $\rm{L}_{10}$ where 
$\rm{L}_{10} = 10^{10} \, \rm{L}_{\odot,B}$ is $10^{10}$ times the blue 
light luminosity of the sun.

We assume that binary coalescences only occur in galaxies.
The absorption-corrected blue light luminosity of a galaxy infers its massive 
star formation and supernova rate which we assume scale with the rate of 
compact binary coalescence within it \cite{Phinney:1991ei}. 
This assumption is well justified when the galaxies reached by the detector 
are dominated by spiral galaxies with ongoing star formation 
(e.g., the Milky Way).
Results papers reporting on S1 and S2 ~\cite{LIGOS1iul, LIGOS2iul, LIGOS2bbh} 
have quoted the upper limit in units of Milky Way Equivalent Galaxy (MWEG) 
which is equivalent to about $1.7 \, \rm{L}_{10}$.
Upper limits on the rate of coalescences calculated during other searches
using S3 and S4 LIGO are given in units of $\rm{L}_{10}$ \cite{LIGOS3S4all}.

We will treat arrival of a gravitational wave at our detectors
as a rare event which can be described by a Poissonian distribution.
The probability of detecting no gravitational waves
(emitted during binary coalescence) with combined SNR greater than
some value $\rho_{c}$ is given by
\begin{eqnarray}
P_{F}(\rho_{c}) = e^{- \nu(\rho_{c})} 
\end{eqnarray}
where $\nu(\rho_{c})$ is the mean number of gravitational wave events
detected with combined SNR greater than $\rho_{c}$ during the
course of a search (e.g., a science run).
We can write $\nu$ more explicitly as the product of 
i) the rate of binary coalescence (per year per $\rm{L}_{10}$),
ii) the total (cumulative) luminousity $C_{L}(\rho_{c})$ (in $\rm{L}_{10}$) 
that the detectors were sensitive to with combined SNR greater than $\rho_{c}$ 
and 
iii) the total observation time $T$ (in years).
We can therefore write
\begin{eqnarray}
P_{F}(\rho_{c}|R,T) = e^{-R \, T \, C_{L}(\rho_{c})}.
\end{eqnarray}
The subscript $F$ stands for foreground and is used to distinguish
this probability from the probability of measuring a background event
with combined SNR greater than $\rho_{c}$ which we shall call
$P_{B}(\rho_{c})$.

The probability of measuring no event candidates 
(true gravitational wave foreground or noise-induced background) 
with combined SNR greater than that of our loudest observed event candidate
$\rho_{c,\rm{max}}$ is given by
\begin{eqnarray}
P(\rho_{c,\rm{max}}|B,R,T) &=& P_{B}(\rho_{c,\rm{max}}) P_{F}(\rho_{c,\rm{max}}) 
\nonumber\\
&=& P_{B}(\rho_{c,\rm{max}}) e^{-R \, T \, C_{L}(\rho_{c,\rm{max}})}.
\end{eqnarray}
We can calculate the probability density as
\begin{eqnarray}
p(\rho_{c,\rm{max}}|B,R,T) &=& \frac{d}{d \rho_{c}} P(\rho_{c,\rm{max}}|B,R,T) \\
&=&
P_{B}^{\prime}(\rho_{c,\rm{max}}) e^{-R \, T \, C_{L}(\rho_{c,\rm{max}})  } 
\times \nonumber \\
& &
\left[
1 + R \, T \, C_{L}(\rho_{c,\rm{max}}) \, \Lambda    
\right]
\end{eqnarray}
where we have defined 
\begin{equation}
  \Lambda =
  \frac{|\mathcal{C}_{L}^{\prime}(\rho_{c,\rm{max}})|}
       {P_{B}^{\prime}(\rho_{c,\rm{max}})}
  \left[
  \frac{\mathcal{C}_{L}(\rho_{c,\rm{max}})}{P_{B}(\rho_{c,\rm{max}})}
  \right]^{-1}
  \, ,
\end{equation}
where the derivatives are with respect to combined SNR $\rho_{c}$.
$\Lambda$ is a measure of the likelihood that the loudest event measured 
during a search is consistent with being a true gravitational wave signal 
(foreground) rather than being caused by noise (background).
We know by definition that the cumulative luminousity $C_{L}(\rho_{c})$ 
our detectors were sensitive to with combined SNR greater than $\rho_{c}$ 
will decrease as $\rho_{c}$ increases and therefore that 
$C_{L}^{\prime}(\rho_{c})$ will always be negative.

Using Bayes' theorem we can find the posterior distribution probability 
distribution of the rate $p(R|\rho_{c,\rm{max}}, T, B)$ using our 
prior knowledge or guess of its distribution $p(R)$ and our
probability distribution $p(\rho_{c,\rm{max}}|B,R,T)$ for the number of 
events exceeding the combined SNR of the loudest measured event:
\begin{eqnarray}
\label{Bayes}
p(R|\rho_{c,\rm{max}}, T, B) = 
\frac{p(R) \, p(\rho_{c,\rm{max}}|B,R,T) }
{\int  p(R) \, p(\rho_{c,\rm{max}}|B,R,T) \, dR  } .
\end{eqnarray}

Since this is the first dedicated search for gravitational waves emitted 
by binaries with spinning component bodies we have no prior knowledge about 
the rate.
To reflect this, we use a uniform prior, $p(R) = \rm{constant}$.
In upper limit calculations for future searches we will be able to use the 
posterior probability distributions calculated for previous searches as our 
prior.
Integrating the denominator of Eq.~(\ref{Bayes}) by parts yields 
\begin{eqnarray}
&\int& p(R) p(\rho_{c,\rm{max}}|B,R,T) dR
\nonumber \\ 
&=& P_{B}^{\prime}(\rho_{c,\rm{max}}) p(R)
\int
e^{-R \, T \, C_{L}(\rho_{c,\rm{max}}) }
\left[
1 + R \, T \, C_{L}(\rho_{c,\rm{max}}) \, \Lambda
\right]
dR \nonumber \\
&=&
- P_{B}^{\prime}(\rho_{c,\rm{max}}) p(R) \frac{1}{T \, C_{L}(\rho_{c,\rm{max}})} 
\left[ 
1 + R \, T \, C_{L}(\rho_{c,\rm{max}}) \, \Lambda + \Lambda
\right]
\end{eqnarray}
where we can take the prior outside the integral since it is
a constant and $P_{B}^{\prime}$ outside the integral since it
will clearly not depend on the rate of true gravitational wave events.
Evaluating the integrand over all possible rates 
(from $R=0$ to $R= \infty$) we find
\begin{eqnarray}
\int_{0}^{\infty} p(R) p(\rho_{c,\rm{max}}|B,R,T) dR
&=& 
P_{B}^{\prime} p(R) \frac{1 + \Lambda}{T \, C_{L}}. 
\end{eqnarray}
In practise we can use a finite upper bound on this integral by choosing
a large value for the rate $R$ with a suitably low probability of occuring. 

Substituting this result back into Bayes' theorem Eq.~(\ref{Bayes})
we find the posterior distrubtion to be:
\begin{eqnarray}
p(R|\rho_{c,\rm{max}}, T, B) 
&=&
e^{-R \, T \, C_{L}} \frac{T \, C_{L}} {1 + \Lambda} 
\left[
1 + R \, T \, C_{L} \, \Lambda
\right]
\end{eqnarray}

To find the upper limit $R_{\alpha}$ on the rate of coalescences 
with confidence $\alpha$ we evaluate
\begin{eqnarray}
\alpha = \int_{0}^{R_{\alpha}} p(R|\rho_{c,\rm{max}}, T, B) \, dR. 
\end{eqnarray}
Integrating by parts yields
\begin{eqnarray}
\label{bayesianprob}
1 - \alpha = e^{-R_{\alpha}\, T \, \mathcal{C}_{L}(\rho_{c,\rm{max}})}
\left[ 1 + \left( \frac{\Lambda}{1+\Lambda} \right) 
\, R_{\alpha}\, T \, \mathcal{C}_{L}(\rho_{c,\rm{max}}) \right].
\end{eqnarray}
The corresponding statistical statement would be that we have 
$\alpha \times 100\%$ confidence that the rate of binary coalescences 
is less than $R_{\alpha}$.

%The upper limit calculations are based on the loudest event 
%statistic~\cite{loudestGWDAW03,ul}, which uses both the detection 
%efficiency at the combined SNR of the loudest event candidate and the 
%associated background probability.

%We evaluate the cumulative luminosity $\mathcal{C}_{L}$ at the combined SNR
%of the loudest coincident trigger seen in this search, 
%$\rho_{c,\rm{max}} = 58.3$  (see Sec.~\ref{sub:results} for discussion of 
%this coincident trigger). 

\subsection{Observation time}
We only use data that was taken during {\it non}-playground times in the
calculation of the upper limit.
The (in-time) non-playground dataset is {\it blinded} in the sense that 
all analysis parameters are tuned and fixed prior to its analysis
in order to avoid statistical bias 
(as described in Secs.~\ref{sec:pipeline})
The observation time $T$ is taken from Table~\ref{tab:analysedtimes},
where we use the {\it non}-playground analyzed times.

\subsection{Calculating the cumulative luminousity}
The cumulative luminosity $\mathcal{C}_{L}(\rho_{c})$ 
to which our search was sensitive to is a function of the detection
efficiency of our search $\mathcal{E}$ and the predicted luminousity $L$ of 
the local universe.

In searches for systems consisting of non-spinning bodies 
detection efficiency $\mathcal{E}$ is found as a function of its chirp mass 
$\mathcal{M} = M \eta^{3/5}$ and effective distance which are combined to 
construct a quantity called the ``chirp distance'' which describes how 
detectable a given source is \cite{systematics, LIGOS3S4all}.
For low values of chirp distance we would expect high detection efficiency
and vice versa. 
We find that the effective distance is not well defined for a source
consisting of spinning bodies and we find an alternative.

For a binary source located at a distance $D$ from a detector, 
the effective distance $D_{\rm eff}$ is the distance at
which it would produce the same SNR if it was positioned directly overhead 
the detector and with optimal orientation 
(i.e., face on to the detector, $\iota=0$) \cite{allen:2005}.
For a system consisting of {\it non}-spinning bodies effective distance can be
calculated using
\begin{eqnarray}
D_{\rm eff} = \frac{D}
{\sqrt{F_+^2 (1 + \cos^{2}\iota)^{2}/4 + F_\times^{2} ( \cos\iota)^2}}
\end{eqnarray}
where $D$ is the distance between the binary and the observer,
$\iota$ is the inclination angle of the binary with respect to the
observer and $F_{+}$ and $F_{\times}$ are the antenna patterns of the detector
(see Eq.~(\ref{Fpluscross})).
The effective distance $D_{\rm eff}$ of a binary will always be
equal or greater than the physical distance $D$.

For a system consisting of spinning bodies, its inclination $\iota$
with respect to a detector will evolve during the course of the inspiral making
the calculation of effective distance complicated (it would in fact be time
dependent if we used the formula above).
Instead, in this search we find efficiency and predicted source luminosity as a
function of the inverse of the {\it expected SNR} of a source.
The expected SNR is defined as the SNR that would be obtained for a given
simulated source assuming we use a template that perfectly matches the emitted
gravitational waveform (i.e., fitting factor $= 1$)
and a detector whose noise power spectrum we can estimate accurately.
We therefore define $\rho_{\rm{expected}} = \left< s,h \right>$ where
$h$ is our template and $s = A h$ is our signal. 
We can calculate the combined expected SNR using the formulas in 
Sec.~\ref{sub:combSNR}.

By taking our distance measure $D_{\rho}$ as the inverse of the expected SNR 
we obtain a quantity which behaves similarly to the chirp distance by taking 
larger values for signals which are louder detectable and by taking smaller 
values as the signals become less detectable.

{\bf define detection efficiency}


We use software injection of simulated signals 
(the target waveforms described in Sec.~\ref{Sec:TargetModel})
to evaluate the efficiency $\mathcal{E}$ for observing an event with combined
SNR greater than $\rho_{c}$, as a function of the source's expected SNR.
We then integrate $\mathcal{E}$ times the predicted source luminosity $L$
as a function of expected SNR and mass.


HERE

\subsection{The likelihood}
The expression for the likelihood $\Lambda$ is
\begin{eqnarray}
  \Lambda =  
  \frac{|\mathcal{C}_{L}^{\prime}(\rho_{c,\rm{max}})|}
       {P_{B}^{\prime}(\rho_{c,\rm{max}})}
  \left[
  \frac{\mathcal{C}_{L}(\rho_{c,\rm{max}})}{P_{B}(\rho_{c,\rm{max}})}
  \right]^{-1}
  \, ,
\end{eqnarray}
where the derivatives are with respect to combined SNR $\rho_{c}$.  
$P_{\rm B}(\rho)$ is the probability that all background coincident triggers 
(as estimated using time-shifts) have a combined SNR less than $\rho$. 
In the case where the loudest event candidate is most likely due to the 
background $\Lambda \rightarrow 0$ and the 
$90\%$ confidence upper limit becomes
\begin{eqnarray}
  R_{90\%} = \frac{2.3}{ T \, \mathcal{C}_{L}(\rho_{c,\rm{max}})} \, .
\end{eqnarray}
In the limit of zero background, i.e., the event is definitely not background, 
$\Lambda \rightarrow \infty$ and the $90\%$ confidence upper limit becomes
\begin{eqnarray}
  R_{90\%} = \frac{3.9}{ T \, \mathcal{C}_{L}(\rho_{c,\rm{max}})} \, .
\end{eqnarray}

For the loudest event candidate in this search we find $P_{\rm B} = 0.23$
and $\Lambda = 0.05$.
{\bf what about CL? does this depend on the sources? should this numbers be pushed
back in the paper too}

Following the tests of the template bank (Sec.~\ref{sub:testingbank}) we also 
know that the efficiency at which we are able to detect sources will depend on 
their spins as well as their effective distance and component masses.
In this upper limit calculation we assess the efficiency of the search using 
software injection of simulated signals representing a population of sources 
with spins randomized so that  
i) the spin magnitude of each of the compact objects is distributed uniformly 
in the range $0 < \chi < 1$ and 
ii) the direction of compact object's spin is uniformly distributed on the 
surface of a sphere. 
%The masses of the sources used to assess the efficiency are in the 
%range $1.0~M_{\odot} < m_{1}, m_{2} < 20.0~M_{\odot}$.
The distances of the simulated sources are chosen uniformly on a logarithmic
scale.
The sky-positions and initial polarization and inclination angles of the 
simulated sources are all chosen randomly and to be uniformly distributed 
on the surface of a sphere.
We evaluated the efficiency of this search for masses in the range 
$1.0~M_{\odot} < m_{1}, m_{2} < 20.0~M_{\odot}$. 
During S3 LIGO's efficiency to binaries in this range was dominated by 
sources within the Milky Way for which detection efficiency was high 
across the the entire mass range investigated due to the proximity of 
these sources Earth. 

The cumulative luminosity function $\mathcal{C}_{L}(\rho_{c})$ can be obtained 
as follows. 
We use software injection of simulated signals 
(the target waveforms described in Sec.~\ref{Sec:TargetModel}) 
to evaluate the efficiency $\mathcal{E}$ for observing an event with combined 
SNR greater than $\rho_{c}$, as a function of the source's expected SNR.
We then integrate $\mathcal{E}$ times the predicted source luminosity $L$ 
as a function of expected SNR and mass.  

The cumulative luminosity as a function of expected SNR can be obtained by 
generating a population of simulated signals using information on the observed 
distribution of sources from standard astronomy catalogs. 
For each simulated signal we calculate the expected SNR as we did when 
assessing the efficiency of the search. 
We use a model based on~\cite{LIGOS3S4Galaxies} for the distribution
of blue light luminosity throughout the nearby Universe. 
Since a binary system will have in general slightly different orientations with 
respect to the two LIGO observatories they will both have slightly different 
expected SNRs.
The efficiency for detection is thus a function of both expected SNRs, and the
integration needed is two-dimensional:
\begin{eqnarray}
  \mathcal{C}_{L}(\rho)=
  \int_0^{\infty} 
  \int_0^{\infty} 
  \mathcal{E}(D_{\rho,\rm{H}},D_{\rho,\rm{L}},\rho) \, 
  L(D_{\rho,\rm{H}}, dD_{\rho,\rm{L}}) \,
  dD_{\rho,\rm{L}} \, dD_{\rho,\rm{H}} 
\end{eqnarray}
where $D_{\rho}$ is the distance measure equal to the inverse of the expected 
SNR, at LHO (H) or LLO (L). 
As mentioned earlier, we evaluate $\mathcal{C}_{L}$ at the combined SNR of our 
loudest event candidate $\rho_{c,\rm{max}} = 58.3$. 

We calculate the upper limit on the rate of coalescence for proto-typical 
NS-BH binaries with masses 
$m_{1} \sim 1.35~M_{\odot}$ and 
$m_{2} \sim 5~M_{\odot}$. 
These values correspond to a population of NS-BH binaries with component 
masses similar to those used to assess the NS-NS and BH-BH upper limits 
in \cite{LIGOS3S4all}. 
To calculate this upper limit we evaluate the efficiency of our search using 
binaries with a Gaussian mass distribution with means, 
$m_{1}= 1.35~M_{\odot}$ and $m_{2} = 5~M_{\odot}$ with standard deviations 
$\sigma_{1}=0.04~M_{\odot}$ and $\sigma_{2} = 1~M_{\odot}$.
%
%The efficiency for this search is computed using a Gaussian mass distribution, 
%with means $m_1 = 1.35 M_{\odot}$, $m_2=5 M_{\odot}$ and standard deviations 
%$\sigma_1 = 0.04 M_{\odot}$, $\sigma_2 = 1 M_{\odot}$.
%These values correspond to a population of NS-BH binaries with component masses 
%similar to  those used to assess the NS-NS and BH-BH upper limits in 
%\cite{LIGOS3S4all}.
%%This choice of masses reflects our expectations about
%%the type of binary systems we believe LIGO is most likely to observe based upon
%%population studies~\cite{Belczynski:2002}.
%%The choice of relatively low component masses also means that our upper limit
%%estimate should be conservative.  
These efficiencies are measured with simulated injected signals, using the 
same pipeline we used to find our candidates, counting the number of 
injections detected with SNR above $\rho_{c,\rm{max}}$, and the number missed. 

Assuming a Gaussian distribution of masses, we obtain an upper limit of 
$\mathcal{R}_{90\%} = 15.8 \,\mathrm{yr}^{-1}\,\mathrm{L_{10}}^{-1}$. 
The upper limit calculation takes into account the possible systematic
uncertainties which 
arise in this search, which are described in some detail in~\cite{systematics},
and we will follow the analysis presented there to calculate the
systematic errors for the above result.  The most significant effects are due 
to the possible calibration inaccuracies of the detectors (estimated using 
hardware injections of simulated signals) and the finite number of Monte Carlo 
injections performed. 

We must also evaluate the systematic errors associated with the chosen 
astrophysical model of potential sources within the galaxy.  We obtain
upper limits on the rate after marginalization over the estimated systematic
errors, as described in~\cite{systematics,ul}. 
After marginalization over these errors we obtain an upper limit of 
$\mathcal{R}_{90\%} = 15.9 \,\mathrm{yr}^{-1}\,\mathrm{L_{10}}^{-1}$.
%Marginalization over these errors causes only a very small (less than $0.5\%$) 
%increase to the upper limit.
 
%We also calculated the upper limits with uniform total mass distribution. 
We also calculate upper limits for a a range of binary systems with 
$m_1 = 1.35 M_{\odot}$ and $m_2$ uniformly distributed between $2$ and 
$20 M_{\odot}$.
These upper limits, both before and after marginalization are shown in 
Fig.~\ref{fig:upperlimit}. 
%It can be seen from this figure that the upper limit decreases as the total 
%mass of the binaries increases. This effect is partially due to improved 
%template bank coverage for heavier asymmetric systems (highest matches for 
%generic spinning systems are obtained for binaries
%with masses $m_1 \simeq 2 M_{\odot}$ and $m_2 \simeq 16 M_{\odot}$, see 
%Sec.~\ref{sub:testingbank}) but
%is primarily caused by the the increase of SNR with total mass 
%($\rho \propto M^{5/6} \eta^{1/2} / d$, see e.g., \cite{thorne.k:1987}).   
%Since systems with {\it higher} SNR are more likely to be detected we are 
%able to place {\it lower} upper limits on the rate of coalescence of these 
%systems in the case where no detection was made.
%During S3 the region of the the Universe from which we would be able to 
%detect binary inspirals was dominated by the Milky Way. 
%Consequently we find that the detection efficiency measured for this search 
%is almost uniform across the range of component masses investigated 
%(i.e., $1.0~M_{\odot} < m_{1}, m_{2} < 20.0~M_{\odot}$).  
%The upper limits calculated are almost constant across the range of masses 
%plotted with a slight increase in the upper limits for binaries with larger 
%total mass where the signals become shorter.

\begin{figure}
\begin{center}
%\includegraphics[width=0.5\textwidth]{Chapter3/Uniform-rate-v-mass_1_100_7_25_2.png}
%\includegraphics[width=0.5\textwidth]{Chapter3/Uniform-rate-v-mass_135_2-20_yrange_1_100.png}
%\includegraphics[width=0.5\textwidth]{Chapter3Uniform-rate-v-mass_135_2-20_yrange_10_20.png}
\includegraphics[width=0.9\textwidth]{Chapter3/Uniform-rate-v-mass_135_2-20_yrange_10_20_dm_45.png}
%\includegraphics[width=0.5\textwidth]{Chpater3/Uniform-rate-v-mass_5_2-20_yrange_1_100.png}
%\end{center}
\caption{Upper limits on the spinning binary coalescence rate per
$\mathrm{L}_{10}$ as a function of the total mass of the binary.
For this calculation, we have evaluated the efficiency of the search
using a population of binary systems with $m_1 = 1.35 M_{\odot}$
and $m_2$ uniformly distributed between $2$ and $20 M_{\odot}$.
The darker area on the plot shows the region excluded after marginalization
over the estimated systematic errors whereas the lighter region shows the
region excluded if these systematic errors are ignored.
The effect of marginalization is typically small ($<1\%$).
The initial decrease in the upper limit corresponds to the increasing
amplitude of the signals as total mass increases.
The subsequent increase in upper limit is due to the counter effect that as
total mass increases the signals become shorter and have fewer cycles in LIGO's
frequency band of good sensitivity.}
\label{fig:upperlimit}
\end{center}
\end{figure}
 


==> Chapter3/dump3 <==
%\label{ch:s3sbbh}
\label{S1ACST}
\label{LNACST}
\label{kappa}
\label{fig:simple_transitional}
\label{alphaf}
\label{fig:orbangmmtm_cone}
\label{apostansatz}
\label{BCV2analysis}
\label{sec:BCV2dtf}
\label{BCV2DTFa}
\label{BCV2DTF}
\label{amp}
\label{sec:maximisation}
\label{basisTemplates}
\label{overlapBasis}
\label{alphaHatMax}
\label{BCV2SNR}
\label{fig:rhosq_hist}
\label{fig:wave_snr}
\label{templatebank}
\label{fig:manifolds}
\label{tmpltbankmetric}
\label{fLSO}
\label{templatebank}
\label{sub:testingbank}
\label{fig:banksims}
\label{phase3.5PN}
\label{psiNM}
\label{sec:pipeline}
\label{fig:pipeline}
\label{fig:sciencesegment}
\label{tab:analysedtimes}
\label{fig:FOMSize_VersusGPS_tmpltbank}
\label{sub:coincAnalysis}
\label{sub:background}
\label{sub:combSNR}
\label{combSNR_2ifo}
\label{combSNR_3ifo}
\label{sub:vetoes}
%\label{slide_trigs}
\label{fig:cum_hist}
\label{fig:snr_snr}
\label{sub:upperlimit}
\label{fig:upperlimit}
    \label{bayesianprob}
\label{xi}
\begin{equation}\label{ul_bg}


==> Chapter3/label3 <==
%\label{ch:s3sbbh}
\label{S1ACST}
\label{LNACST}
\label{kappa}
\label{fig:simple_transitional}
\label{alphaf}
\label{fig:orbangmmtm_cone}
\label{apostansatz}
\label{BCV2analysis}
\label{sec:BCV2dtf}
\label{BCV2DTFa}
\label{BCV2DTF}
\label{amp}
\label{sec:maximisation}
\label{basisTemplates}
\label{overlapBasis}
\label{alphaHatMax}
\label{BCV2SNR}
\label{fig:rhosq_hist}
\label{fig:wave_snr}
\label{templatebank}
\label{fig:manifolds}
\label{tmpltbankmetric}
\label{fLSO}
\label{templatebank}
\label{sub:testingbank}
\label{fig:banksims}
\label{phase3.5PN}
\label{psiNM}
\label{sec:pipeline}
\label{fig:pipeline}
\label{fig:sciencesegment}
\label{tab:analysedtimes}
\label{fig:FOMSize_VersusGPS_tmpltbank}
\label{sub:coincAnalysis}
\label{sub:background}
\label{sub:combSNR}
\label{combSNR_2ifo}
\label{combSNR_3ifo}
\label{sub:vetoes}
\label{sub:results}
%\label{slide_trigs}
\label{fig:cum_hist}
\label{fig:snr_snr}
\label{sub:upperlimit}
\label{fig:upperlimit}
    \label{bayesianprob}
\label{xi}
\begin{equation}\label{ul_bg}


==> Chapter5/ParamEst.tex <==
%$Id: ParamEst.tex,v 1.1.1.1 2007-10-26 15:41:53 spxgwj Exp $

\chapter{Parameter Estimation}
\label{ch:param}

\section{Decoupling of amplitude and phase terms}

Consider the following waveform defined in the frequency domain:
\begin{eqnarray}
h(f) = G(\alpha_{j}) e^{i \psi(m_{1}, m_{2})}.
\end{eqnarray}

To construct the Fisher matrix we must calculate various derivatives:
\begin{eqnarray}
\frac{\partial h(f)}{\partial \alpha_{j}} = 
\frac{\partial G(\alpha_{j})}{\partial \alpha_{j}} 
e^{i \psi(m_{1}, m_{2})}
\end{eqnarray}
and
\begin{eqnarray}
\frac{\partial h(f)}{\partial m_{j}} = 
G(\alpha_{j}) i 
\frac{\partial \psi(m_{1}, m_{2}))}{\partial m_{j}}
 e^{i \psi(m_{1}, m_{2})}.
\end{eqnarray}
If the functions $G(\alpha_{j})$ and $\psi(m_{1}, m_{2}))$ are wholly real 
we will find that the Fisher matrix elements corresponding to derivatives 
with respect to amplitude and phasing coefficients will decouple from each 
other:
\begin{eqnarray}
\left( \frac{\partial h}{\partial \alpha_{j}} | \frac{\partial h}{\partial m_{j}} \right)
= 
\Re \int \frac{\partial G(\alpha_{j})}{\partial \alpha_{j}} i
\frac{\partial \psi(m_{1}, m_{2}))}{\partial m_{j}} \frac{df}{S_{n}(f)}
= 0.
\end{eqnarray}
This will yield a block diagonal Fisher matrix (one block corresponding to inner
products of derivatives with respect to amplitude coefficients and the other 
corresponding to the inner products of derivatives with respect to phase 
coefficients) which upon inversion will lead to a block diagonal covariance
\footnote{It is trivial to show that the inverse of a block diagonal matrix
is also block diagonal. Both matrices will have the same elements set to zero} 
matrix (one block corresponding to the variances and covariances of the 
amplitude coefficients and the other corresponding to the variances and 
covariances of the phase coefficients).


\section{Error propagation}
We make use of the error propagation formula
\begin{eqnarray}
\delta f(x_{1}, x_{2} \ldots x_{n})
= \left( \sum_{i}^{n} \sum_{j}^{n} \left( \frac{\partial f}{\partial x_{i}}  \frac{\partial f}{\partial x_{j}} C_{ij}  \right) \right)^{1/2}
\end{eqnarray}
where $C$ is the covariance matrix.  




==> Introduction/cite1 <==
%In 1905 Einstein published the Special Theory of Relativity (SR) \cite{einstein-1920}. In it he 
(Following Hartle \cite{Hartle} Chapter 23, Schutz \cite{Schutz} Chapter 9,
Hakim \cite{Hakim} Chapter 8,
d'Inverno \cite{inverno} Chapter 20 and  
Misner, Thorne and Wheeler \cite{MTW}) Chapter 36.
d'Alembertian (Eq.~({\ref{dalembertian}})) \cite{GreenWave} which will yield 
as $T^{\alpha \beta}_{\phantom{\alpha \beta}, \beta} = 0$ \cite{Hartle}.
From dimensional analysis (see e.g. Hartle \cite{Hartle} Chapter 23)
$\rv \equiv \xv_{1} - \xv_{2}$ \cite{LL}.
centre of mass at position $\rv \equiv \xv_{1} - \xv_{2}$ \cite{LL}.}
\item ref LIGO-GEO paper \cite{abbott-2004-517} for technical details
Damour et al. (2001) \cite{DIS2001}.
(available on Virgo home page \cite{VirgoHomePage}).
The EGO noise curve is given by Van Den Broeck and Sengupta (2007) \cite{broeck-2007-24}.
The LISA noise curve is given by Barack and Cutler (2004) \cite{barack:082005}.
\cite{abbott-2004-517}.
\cite{LIGOS1iul}
%{\bf !!In \cite{arun:084008} intro detection methods for different 
(see, for example, Whalen (1971) \cite{whalen:1971}).
Following the derivation in Section 2A of Finn (1992) \cite{Finn92} we
%Note that this definition (from \cite{arun:084008}, Eq.~(2.10)) is equivalent 
%in Eq.~(2.21) of \cite{Finn92} when $g(t)$ and $h(t)$ are real.
(i.e., when $S_{n}(f)$ is small) \cite{babak:2006}.
%and refer to Babak et al. (2006) \cite{babak:2006}}
From \cite{whalen:1971}.
%Following \cite{whalen:1971} we consider a region $A$ containing possible values
Following \cite{whalen:1971} (Eqs. (1.12-1.14)) we find that 
Following the derivation in \cite{whalen:1971} (Eqs. (4.26-4.28)) 


==> Introduction/dump1 <==
\label{ch:intro}
%\begin{equation} \label{strain}
\label{EEgen}
\label{curvtensor}
\label{spacetimemetric}
\label{metricg}
\label{riccifull}
\label{christg}
\label{christh}
\label{riccih}
\label{tracereverse}
\label{einsteinCurvatureFull}
%\label{dalembertian}
%\label{vdef}
\label{coordtrans}
\label{gaugetrans}
\label{gaugetranstrace}
\label{gaugetranstr}
\label{sec:lorentzgauge}
%\label{lorentzgauge}
\label{lorentzgauge}
\label{dalembertian}
\label{boxhbar}
\label{hbarwave}
\label{firstrel}
\label{secondrel}
\label{sec:applyingTT}
\label{xiwave}
\label{metricTT}
\label{EEsource}
\label{energymmtm}
\label{GreenSoln}
\label{barhfarzone}
\label{TijInt}
\label{quadmassmoment}
\label{metricquad}
\label{strainform} 
\label{strainvalue}
\label{one_body}
\label{binaryh}
\label{sec:detection}
\label{timedepL}
\label{genstrain}
\label{dscross}
\label{test_masses}
\label{ifo_detection_1}
%\label{interferometer}
\label{PSDcurves_all}
\label{sec:DA}
\label{inner_any}
\label{inner_real_BCV}
\label{inner_real_AISS}
\label{matchedfilterresponse}
\label{gaussianresponse}
\label{lintrans}

